User Agency and System Automation in Interactive Intelligent Systems

Balancing user agency and system automation is essential for effective human-AI interactions. Fully automated systems can deliver efficiency but risk undermining usability and user autonomy, while purely manual tools are often inefficient and fail to enhance user capabilities. This dissertation addresses the question: "How can we balance user agency and system automation for interactions with intelligent systems?" We present four main contributions. First, we develop a spherical electromagnet that provides adjustable forces on an untethered tool, allowing haptic feedback while preserving user agency. Second, we create an integrated sensing and actuation system that tracks a passive magnetic tool in 3D and delivers haptic feedback without external tracking. Third, we propose an optimal control method for electromagnetic haptic guidance that balances user input with system control, enabling users to adjust trajectories and speed. Finally, we introduce a model-free reinforcement learning approach for adaptive interfaces that learns interface adaptations without heuristics or real user data. Our simulations and user studies show that shared control significantly outperforms naive strategies. By incorporating explicit or implicit models of human behavior into control strategies, intelligent systems can better account for user agency. We demonstrate that the trade-off between agency and automation is both an algorithmic challenge and an engineering concern, shaped by the design of physical devices and user interfaces. We advocate an integrated, end-to-end approach-combining algorithmic, engineering, and design perspectives-to enable more intuitive and effective interactions with intelligent systems.

==> chapters/01_introduction/content/thesis_statement.tex <==
\section{Thesis Statement}
% In this thesis, we propose \textbf{\method{} as a computational framework for adaptive UIs}.
% By implicitly considering the closed-loop, iterative nature of HCI, \method{} extends existing AUIs by enabling \textbf{permanent and effective adaptation of input and output mechanisms}.
% % \\ \\
% \noindent
% In three case studies, we have demonstrated that \method{} methods \textbf{improve the usability of emerging technologies} by assisting users in accomplishing their high-level goals.
% We have shown that model predictive control supports users in a challenging creative robotic task.
% In addition, we demonstrated that reinforcement learning can learn individual cooperative policies solely by observing a user's gaze interactions with a UI. 
% Finally, we proposed a cognitively plausible hierarchical reinforcement learner that reproduces human task interleaving, being applicable in various HCI tasks.

==> chapters/04_joint_interfaces/contact_free/sections/00_abstract.tex <==
% !TeX root = ../main.tex

\begin{abstract}
%\TL{Page limit is 7. inc references.}
%\remove{In this paper we introduce a novel contact-free volumetric haptic feedback device. A symmetric electromagnet is used in combination with a dipole magnet model and a simple control law to deliver dynamically adjustable forces onto a hand-held tool such as a stylus. The tool can be 3D printed and only requires an embedded permanent magnet and thus can be entirely untethered. The force, however, while contact-free, remains grounded via the spherical electromagnet and hence relatively large forces (1N at a 3cm distance) can be felt by the user. The device is capable of rendering both attractive and repulsive forces in a thin shell. While the hardware is custom-built, it consists only of readily available components and we will release all soft- and hardware designs to foster future research. We report findings from a user experiment with 6 participants, characterizing force delivery aspects and perceived precision of our system. We found that, that our system has resolution of at least 25 user discernable locations, for repelling forces, distributed across the hemisphere. }

%\suggestion{

%}
\end{abstract}

% \begin{IEEEkeywords}
% %IEEE, IEEEtran, journal, \LaTeX, paper, template.
% spherical electromagnet, magnetic dipoles, force feedback, hand-tool, grounded haptics.
% \end{IEEEkeywords}


%%%%%%
%%%%%%
%% Problem: 
%%  - wireless hand-tool input devices, like mouses and pointers, does not provide haptic feedback forces; 
%%  - while available haptic manipulators needs a mechanical physic chain to control the movement of a holding tool.
%%  - haptic feedback forces are desired to enhance the user experience of physical virtual objects, 
%% - and to enable new modes of multi modal interaction: similar to the clicking or press-key-down sensations.
%%
%% Our approach:
%%  - System: 
%%      - electromagnet, magnetic forces, 
%%      - spherical symmetry, 3 DoF (novel geometry)
%%      - no moving parts on the actuator side, only the hand-tool
%%      - Easy and affordable to fabricate (significance to haptic community) 
%%       - Off-the-shelf electronics
%%      - self-contained input/output, 
%%      - user-in-the-loop control, 
%%      - Modelling:
%%          - Model of B, force and torque given actuation/current
%%          - Non-linear optimization method for tool position estimation given N hall sensors
%%  - Interactions: 
%%      - desktop input/output tool-based
%%      - tool tracking and force feedback, 
%%      - graspable haptics
%%      - untethered, midair feedback
%%      - hot-swappable, exchangeable tool
%%      - applicable to wearable haptics thimble or gloves in certain actuation volume
%%      - grounded forces even if no mechanical link (magnetic action/reaction forces)
%%      - from DC forces to vibration
%%      - User evaluation (JNDs) for,
%%          - perceived forces, 
%%          - positioning resolution
%%  - Applications envision/validation: 
%%      - haptic/tangible complement to
%%          - Spherical displays
%%          - shape changing interfaces
%%      - Desktop handle input with haptic feedback
%%      - virtual surfaces/volumes in VR/AR
%%      - 3D design
%%      - Education, haptic training
%%      - Teleoperation, medical
%%      - Gaming
%%
%%  Conclusions: 
%%  - our affordable, self-contained haptic device with spherical geometry enable simple yet convincing haptics feedback forces.
%%  - user test shows that our systems enables to distinguish attractor/repulsive points, geometrical shapes 
%%  - we demonstrate few applications as desktop device and in VR.

%%% Abstract:
%% Contribution 1st statement:
%We introduce an air-gapped haptic interaction system with user-in-the-loop control for unexplored spherical geometry.  
%WHat it does from a user perspective:

%%% Title ideas
% magnet, coils, electricial, for? use?
% sphere
% 3D
% airgapped
% controllable
% novel
% actuator
% stand-alone
% electromagnetic
% haptic 
% user-in-the-loop
% wireless
% contact-free
% passive tools
% non-planar
% in-air
% controllable 
% sensing and action


==> chapters/04_joint_interfaces/contact_free/sections/01_introduction.tex <==
% !TeX root = ../main.tex

\section{Introduction}
Many emerging computing paradigms such as virtual and augmented reality (VR/AR) rely on haptic feedback as an additional information channel to improve the user experience. For example, in VR, haptic feedback increases the sense of presence and immersion by rendering collisions, shapes, and forces between the user and virtual objects.

Existing approaches either rely on vibro-tactile actuators that are embedded into handheld controllers, displays or worn on the body. Such actuators can only render coarse, non-localized haptic sensations. More complex setups such as articulated arms and exoskeletons can render both large-force haptic feedback and can operate in three-dimensional space, but typically require force anchoring in the environment and require complex, and often bulky mechanisms, which prevents walk-up-and-use scenarios, thus hindering user uptake.  

To address this challenge, we propose an approach to deliver contact-free, volumetric haptic feedback via an omni-directional electromagnet. The device consists of a single 60 mm diameter spherical electromagnet and can render attractive and repulsive forces onto permanent magnets embedded in pointing tools such as a stylus or magnets directly worn on the user's fingertip. Leveraging a dipole-dipole approximation of the electromagnet-magnet interaction, our system is capable of calculating and controlling the forces exerted onto the permanent magnet in real-time while dynamically adjusting the force that is perceived by the user. The system can deliver perceptible forces up to 1N in a thin volume above the surface. Furthermore we demonstrate that users can distinguish at least 25 different set-points separated by 18$^\circ$ on the surface of the sphere. %In this work we focus on the control of 3 DoF forces. However, the interaction between magnets does not only involve forces but also torques which could be controlled in the same manner as presented here. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{\dir/contact_free/figures/teaser_v2.png}
    \caption{We introduce a novel contact-free mechanism to render haptic feedback onto a tracked stylus via a hemispherical electromagnet. An approximate model of the magnet interaction and a computationally efficient control strategy allow for the dynamic rendering of  attracting and repulsive forces, for example, allowing users to explore virtual surfaces in a thin shell surrounding the device (inset).}
    \label{fig:syst_overview}
\end{figure}{} 

To demonstrate the efficacy of our approach we designed a functional prototype comprising of an iron core and three custom wound copper coils. The electromagnet is encased in a plastic dome upon which tools can come into contact and move about its surface (see \figref{fig:syst_overview}). The prototypical system can render radial (along the vector from the magnet to the tool) and tangential forces, both in the attractive and repulsive polarity. The system can furthermore dynamically adjust the opening angle and steepness of the electromagnetic potential to
%form perceivable hills and valleys respectively (see \figref{fig:syst_overview}, inset). For example,
 gently guide the user towards a desired set-point in the thin volume above the device.    

Modulating the magnetic field as a function of tool position opens the door to many different interactive applications. In a virtual terrain exploration, the tool can be repelled when moved along mountains and attracted to valleys while descending (see \figref{fig:syst_overview}, inset). As another example, the sensation of stirring a viscous liquid may be created by emulating the drag of the fluid on the tool. To enable these interactive experiences, our device builds on three key components that represent our contributions in this work:
\begin{itemize}
    \item A computational model based on magnetic dipole-dipole interaction to produce force maps that allow for designing and generating location-dependent feedback, 
    \item The design and implementation of a 3 degree-of-freedom (DoF) spherical electromagnet prototype,
    \item A control strategy that translates desired high-level forces into low-level input signals (currents/voltages) for the coils, fast enough for interactive use.
\end{itemize}

To assess the efficacy of the proposed design we characterize the system properties experimentally and report findings from a perceptual study which explores the thresholds for perception and localization capabilities of the electromagnetic actuation approach. Results from these early user tests indicate that users can perceive at least 25 different spatial locations with high precision.  



%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%
%Many VR systems leverage vibro-tactile actuators, embedded in hand-held controllers (e.g., HTC Vive),  displays \cite{Wellman1995} or worn on the body \cite{Cybertouch, Gloveone}. This feedback modality  can only offer coarse, non-localized haptic sensation. More complex setups often involving articulated arms or external braking mechanisms \cite{Massie94, Stamper1997, VanDerLinde2002, Araujo2016} can reproduce higher fidelity haptics and render both tactile and kinesthetic feedback. While such approaches can produce large forces, they are not suitable for mobile scenarios due to their mechanical constraints.

%The sense of touch is vital for interacting with real-world objects. It not only allows us to judge materials, physical properties and constraints; it also allows us to manipulate the objects precisely. However, digital objects lack the physical presence and therefore cannot be touched, perceived or manipulated to a satisfactory and accurate level. This lack greatly reduces the immersion of digital environments. Especially with the rise of Virtual- and Augmented-Reality the haptic perception of virtual objects has gained tremendous importance. 

%Due to this, it is not surprising that a large variety of haptic interfaces exist. [name some]. However, these often operate on a plane surface [cite, cite, cite]. This limits the possible applications, especially since many real-world objects are not constrained to a planar surface. Another branch of haptic research focuses on volumetric haptic devices, which are capable of operating in a three dimensional space [some more citations]. However, these are often constrained by tools integrated with the device; thereby eliminating the potential of swapping tools on the fly and decreasing the immersion for the user. 

%To address these limitations, we introduce \devicename{}, a stand-alone haptic device capable of contact-free volumetric input sensing and rendering of nonplanar haptic forces. Our novel approach is based on the core principles of electromagnetism. We introduce a spherical electromagnet, consisting of three orthogonal coils. The advantage of using an electromagnet is that they are accurately controllable and do not require a physical link to exert force on an object. By controlling the current in each coil separately we can precisely render a force towards the center of the magnet over a distance. The second electromagnetic principle we employ is the hall effect to measure the magnetic field. We add a simple permanent magnet to a tool. By accurately modelling the electromagnetic field of the actuator and subtracting this from our sensor readings, we can triangulate the remaining field and thereby determine the position of the tool (permanent magnet). 

%Next to our hardware contribution, we layout an analytical model for calculating the force of the electromagnet on a permanent magnet given relative orientation. Similarly we introduce a non-linear problem to determine the position of a magnet in space. We solve this problem using an off-the-shelf solver in sub millisecond time. Finally, we introduce a mapping of desired forces with regard to current tool position and desired tool position. 

%We characterize the positioning, resolution and perceived forces of our system in a just-noticable-difference study (JND). We also show possible application domains, such as ..., ... and ....

%\devicename{} is easy and afforable to fabricate. To encourage adaption and exploration of this system. We make all the source code, blueprints and fabrication instructions freely available. 

% Problem:
% \begin{itemize}
%     \item ...
% \end{itemize}


% Hardware:
% \begin{itemize}
% \item Novel Hardware
%   \item Stand alone system
%   \item user-in-the-loop haptic feedback
%   \item easy and affordable to fabricate
%   \item Off-the-shelf electronics
%   \item hot-swappable 
% \end{itemize}

% Modelling:
% \begin{itemize}
%     \item Model of B, force and torque given actuation/current
%     \item Non-linear optimization method for determine permanent magnet in 3D space given N sensors
% \end{itemize}

% Evaluation:
% \begin{itemize}
%     \item Just Noticeable Difference (JND)
% \end{itemize}

==> chapters/04_joint_interfaces/contact_free/sections/macros_cmds.tex <==


%Shorthand for consistent references

%variables from magpen
% \newcommand{\RmagtopenBold}{\mathbf{r_{mp}}}
% \newcommand{\RmagtopenBoldt}{\mathbf{\Tilde{r}_{mp}}}
% \newcommand{\Rmagtopen}{r_{mp}}
% \newcommand{\Rmagtopent}{\Tilde{r}_{mp}}
% %\newcommand{\mpBold}{\mathbf{m_p}}
% \newcommand{\mpBoldt}{\mathbf{\Tilde{m}_{p}}}
% \newcommand{\mmBold}{\mathbf{m_m}}
% \newcommand{\posm}{\mathbf{p_m}}
% \newcommand{\posp}{\mathbf{p_p}}
% \newcommand{\posst}{\mathbf{s}(\theta)}
% \newcommand{\ed}{\mathbf{e_d}}
% \newcommand{\et}{\mathbf{e_t}}
% \newcommand{\ez}{\mathbf{e_z}}
% \newcommand{\Rtheta}{\mathbf{r_{\theta}}}
% \newcommand{\Cost}{\mathcal{C}}
% \newcommand{\stheta}{\sin{\angt}}
% \newcommand{\ctheta}{\cos{\angt}}
% \newcommand{\sphi}{\sin{\angp}}
% \newcommand{\cphi}{\cos{\angp}}
% \newcommand{\angt}{\beta}
% \newcommand{\angp}{\gamma}



==> chapters/04_joint_interfaces/contact_free/sections/zz_applications.tex <==
% \section{Further Applications}
% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{example-image}
%     \caption{Some sub figure with different use cases}
%     \label{fig:my_label}
% \end{figure}{}

A cornucopia of possible applications exists for \devicename{}. We show three different applications in Virtual reality.



% Uses:
% \begin{itemize}
%     \item desktop input/output
%     \item tangible, virtual, midair surfaces and volumes
%     \item tool base (ex. stylus) or wearable (thimble)
% \end{itemize}

% Existing work:
% \begin{itemize}
%     \item spherical displays
%     \item shape changing interfaces
%     \item levitated handles
%     \item tangible interfaces 
% \end{itemize}{}

% Scenarios:
% \begin{itemize}
%     \item VR/AR/MR
%     \item training/eduction
%     \item 3D design
%     \item Gaming
% \end{itemize}{}

==> chapters/04_joint_interfaces/contact_free/sections/zz_not_used_bib.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Biblio Magpen %%%%%
@article{lam2013model,
  title={Model predictive contouring control for biaxial systems},
  author={Lam, Denise and Manzie, Chris and Good, Malcolm C},
  journal={IEEE Transactions on Control Systems Technology},
  volume={21},
  number={2},
  pages={552--559},
  year={2013},
  publisher={IEEE}
}
@article{yung1998analytic,
  title={An analytic solution for the force between two magnetic dipoles},
  author={Yung, Kar W and Landecker, Peter B and Villani, Daniel D},
  journal={Physical Separation in Science and Engineering},
  volume={9},
  number={1},
  pages={39--52},
  year={1998},
  publisher={Hindawi}
}


@INPROCEEDINGS{Faulwasser:2009,
author={T. Faulwasser and B. Kern and R. Findeisen},
booktitle={Proceedings of the 48h IEEE Conference on Decision and Control (CDC)},
title={Model predictive path-following for constrained nonlinear systems},
year={2009},
pages={8642-8647},
doi={10.1109/CDC.2009.5399744},
ISSN={0191-2216},
month={Dec},
}

@inproceedings{Mueller2013,
author = {Mueller, M.W. and D'Andrea, R.},
booktitle = {Proceedings of the European Control Conference (ECC), 2013},
isbn = {9783952417348},
mendeley-groups = {Trajectory generation},
pages = {1383--1389},
title = {{A model predictive controller for quadrocopter state interception}},
url = {http://ieeexplore.ieee.org/xpls/abs\_all.jsp?arnumber=6669415},
year = {2013}
}

@article{kloosterman2009systematic,
  title={Systematic review of the effects of exercise therapy on the upper extremity of patients with spinal-cord injury},
  author={Kloosterman, MGM and Snoek, GJ and Jannink, MJA},
  journal={Spinal cord},
  volume={47},
  number={3},
  pages={196},
  year={2009},
  publisher={Nature Publishing Group}
}

@article{AGUIAR2008,
title = "Performance limitations in reference tracking and path following for nonlinear systems",
journal = "Automatica",
volume = "44",
number = "3",
pages = "598 - 610",
year = "2008",
issn = "0005-1098",
doi = "10.1016/j.automatica.2007.06.030",
url = "http://www.sciencedirect.com/science/article/pii/S0005109807003482",
author = "A. Pedro Aguiar and Joao P. Hespanha and Petar V. Kokotovic",
}

@article{Liniger2014,
author = {Liniger, Alexander and Domahidi, Alexander and Morari, Manfred},
doi = {10.1002/oca.2123},
file = {:D$\backslash$:/Mendeley/Liniger, Domahidi, Morari - 2014 - Optimization-based autonomous racing of 143 scale RC cars.pdf:pdf},
issn = {01432087},
journal = {Optimal Control Applications and Methods},
keywords = {autonomous racing,drift control,fast model predictive control,model predictive control,nonlinear,nonlinear receding horizon control,vehicle control},
mendeley-groups = {Trajectory generation},
title = {{Optimization-based autonomous racing of 1:43 scale RC cars}},
url = {http://doi.wiley.com/10.1002/oca.939},
year = {2014}
}

@article{dasilva:2008:mpc,
author = {Da Silva, M. and Abe, Y. and Popović, J.},
title = {Simulation of Human Motion Data using Short-Horizon Model-Predictive Control},
journal = {Computer Graphics Forum},
volume = {27},
number = {2},
pages = {371-380},
keywords = {I.3.7 Computer Graphics, Three Dimensional Graphics and Realism Animation},
doi = {10.1111/j.1467-8659.2008.01134.x},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/j.1467-8659.2008.01134.x},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1111/j.1467-8659.2008.01134.x},
year = {2008},
}

@article{Gebhardt:2018,
	author = {Gebhardt, Christoph and Stevsic, Stefan and Hilliges, Otmar},
	title = {{Optimizing for Aesthetically Pleasing Quadrotor Camera Motion}},
	journal = {ACM Transactions on Graphics (Proceedings of ACM SIGGRAPH)},
	issue_date = {August 2018},
	volume = {37},
	number = {4},
	month = august,
	year = {2018},
	pages = {90:1--90:11},
	articleno = {90},
	numpages = {11},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@misc{domahidi2014forces,
  title={FORCES Professional. embotech GmbH (http://embotech. com/FORCES-Pro)},
  author={Domahidi, Alexander and Jerez, Juan},
  year={2014},
  publisher={July}
}
@incollection{hart1988development,
  title={Development of NASA-TLX (Task Load Index): Results of empirical and theoretical research},
  author={Hart, Sandra G and Staveland, Lowell E},
  booktitle={Advances in psychology},
  volume={52},
  pages={139--183},
  year={1988},
  publisher={Elsevier}
}

@online{Sensel2019,
author ={{Sensel Inc.}},
year = {2019},
title ={Sensel | Interaction evolved},
url ={https://sensel.com/},
month ={Jan},
lastaccessed ={Jan 2, 2019},
}

@inproceedings{Aksan:2018:DeepWriting,
  author = {Aksan, Emre and Pece, Fabrizio and Hilliges, Otmar},
  title = {{DeepWriting: Making Digital Ink Editable via Deep Generative Modeling}},
  booktitle = {SIGCHI Conference on Human Factors in Computing Systems},
  series = {CHI '18},
  year = {2018},
  location = {Montr{\'}eal, Canada},
  publisher = {ACM},
  address = {New York, NY, USA},
}

@article{zitnick2013handwriting,
  title={Handwriting beautification using token means},
  author={Zitnick, C Lawrence},
  journal={ACM Transactions on Graphics (TOG)},
  volume={32},
  number={4},
  pages={53},
  year={2013},
  publisher={ACM}
}



@inproceedings{poupyrev2004haptic,
  title={Haptic feedback for pen computing: directions and strategies},
  author={Poupyrev, Ivan and Okabe, Makoto and Maruyama, Shigeaki},
  booktitle={CHI'04 extended abstracts on Human factors in computing systems},
  pages={1309--1312},
  year={2004},
  organization={ACM}
}

@inproceedings{lee2004haptic,
  title={Haptic pen: a tactile feedback stylus for touch screens},
  author={Lee, Johnny C and Dietz, Paul H and Leigh, Darren and Yerazunis, William S and Hudson, Scott E},
  booktitle={Proceedings of the 17th annual ACM symposium on User interface software and technology},
  pages={291--294},
  year={2004},
  organization={ACM}
}

@article{kyung2008haptic,
  title={Haptic stylus and empirical studies on braille, button, and texture display},
  author={Kyung, Ki-Uk and Lee, Jun-Young and Park, Junseok},
  journal={BioMed Research International},
  volume={2008},
  year={2008},
  publisher={Hindawi Publishing Corporation}
}

@article{withana2010impact,
  title={ImpAct: Immersive haptic stylus to enable direct touch and manipulation for surface computing},
  author={Withana, Anusha and Kondo, Makoto and Makino, Yasutoshi and Kakehi, Gota and Sugimoto, Maki and Inami, Masahiko},
  journal={Computers in Entertainment (CIE)},
  volume={8},
  number={2},
  pages={9},
  year={2010},
  publisher={ACM}
}

@inproceedings{iwata1993pen,
  title={Pen-based haptic virtual environment},
  author={Iwata, Hiroo},
  booktitle={Virtual Reality Annual International Symposium, 1993., 1993 IEEE},
  pages={287--292},
  year={1993},
  organization={IEEE}
}

@inproceedings{kyung2009precise,
  title={Precise manipulation of GUI on a touch screen with haptic cues},
  author={Kyung, Ki-Uk and Lee, Jun-Young and Srinivasan, Mandayam A},
  booktitle={EuroHaptics conference, 2009 and Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems. World Haptics 2009. Third Joint},
  pages={202--207},
  year={2009},
  organization={IEEE}
}

@inproceedings{pangaro2002actuated,
  title={The actuated workbench: computer-controlled actuation in tabletop tangible interfaces},
  author={Pangaro, Gian and Maynes-Aminzade, Dan and Ishii, Hiroshi},
  booktitle={Proceedings of the 15th annual ACM symposium on User interface software and technology},
  pages={181--190},
  year={2002},
  organization={ACM}
}

@inproceedings{yoshida2006proactive,
  title={Proactive desk II: Development of a new multi-object haptic display using a linear induction motor},
  author={Yoshida, Shunsuke and Noma, Haruo and Hosaka, Kenichi},
  booktitle={Virtual Reality Conference, 2006},
  pages={269--272},
  year={2006},
  organization={IEEE}
}


@inproceedings{kim2008digital,
  title={Digital rubbing: playful and intuitive interaction technique for transferring a graphic image onto paper with pen-based computing},
  author={Kim, Hyunjung and Kim, Seoktae and Lee, Boram and Pak, Jinhee and Sohn, Minjung and Lee, Geehyuk and Lee, Woohun},
  booktitle={CHI'08 Extended Abstracts on Human Factors in Computing Systems},
  pages={2337--2342},
  year={2008},
  organization={ACM}
}

@inproceedings{bau2010teslatouch,
  title={TeslaTouch: electrovibration for touch surfaces},
  author={Bau, Olivier and Poupyrev, Ivan and Israr, Ali and Harrison, Chris},
  booktitle={Proceedings of the 23nd annual ACM symposium on User interface software and technology},
  pages={283--292},
  year={2010},
  organization={ACM}
}

@inproceedings{cho2016realpen,
  title={RealPen: Providing Realism in Handwriting Tasks on Touch Surfaces using Auditory-Tactile Feedback},
  author={Cho, Youngjun and Bianchi, Andrea and Marquardt, Nicolai and Bianchi-Berthouze, Nadia},
  booktitle={Proceedings of the 29th Annual Symposium on User Interface Software and Technology},
  pages={195--205},
  year={2016},
  organization={ACM}
}

@inproceedings{jansen2010mudpad,
  title={MudPad: tactile feedback and haptic texture overlay for touch surfaces},
  author={Jansen, Yvonne and Karrer, Thorsten and Borchers, Jan},
  booktitle={ACM International Conference on Interactive Tabletops and Surfaces},
  pages={11--14},
  year={2010},
  organization={ACM}
}

@article{buxton1985issues,
  title={Issues and techniques in touch-sensitive tablet input},
  author={Buxton, William and Hill, Ralph and Rowley, Peter},
  journal={ACM SIGGRAPH Computer Graphics},
  volume={19},
  number={3},
  pages={215--224},
  year={1985},
  publisher={ACM}
}

@article{norman1999affordance,
  title={Affordance, conventions, and design},
  author={Norman, Donald A},
  journal={interactions},
  volume={6},
  number={3},
  pages={38--43},
  year={1999},
  publisher={ACM}
}

@book{dessoir1892hautsinn,
  title={{\"U}ber den Hautsinn},
  author={Dessoir, Max},
  year={1892}
}

@article{gibson1966senses,
  title={The senses considered as perceptual systems.},
  author={Gibson, James Jerome},
  year={1966},
  publisher={Houghton Mifflin}
}

@article{robles2001force,
  title={Force can overcome object geometry in the perception of shape through active touch},
  author={Robles-De-La-Torre, Gabriel and Hayward, Vincent},
  journal={Nature},
  volume={412},
  number={6845},
  pages={445},
  year={2001},
  publisher={Nature Publishing Group}
}

@incollection{robles2008principles,
  title={Principles of haptic perception in virtual environments},
  author={Robles-De-La-Torre, Gabriel},
  booktitle={Human haptic perception: Basics and applications},
  pages={363--379},
  year={2008},
  publisher={Springer}
}

@article{robles2006importance,
  title={The importance of the sense of touch in virtual and real environments},
  author={Robles-De-La-Torre, Gabriel},
  journal={Ieee Multimedia},
  volume={13},
  number={3},
  pages={24--30},
  year={2006},
  publisher={IEEE}
}

@article{cole1995living,
  title={Living without touch and peripheral information about body position and movement: Studies with deafferented subjects},
  author={Cole, Jonathan and Paillard, Jacques},
  journal={The body and the self},
  pages={245--266},
  year={1995},
  publisher={MIT Press Cambridge, MA}
}

@article{johansson1992somatosensory,
  title={Somatosensory control of precision grip during unpredictable pulling loads},
  author={Johansson, Roland S and H{\"a}ger, Charlotte and Riso, Ronald},
  journal={Experimental brain research},
  volume={89},
  number={1},
  pages={192--203},
  year={1992},
  publisher={Springer}
}

@article{finley2005surgical,
  title={Surgical robotics},
  author={Finley, David S and Nguyen, Ninh T},
  journal={Current surgery},
  volume={62},
  number={2},
  pages={262--272},
  year={2005},
  publisher={Elsevier}
}

@article{van2009value,
  title={The value of haptic feedback in conventional and robot-assisted minimal invasive surgery and virtual reality training: a current review},
  author={Van der Meijden, OAJ and Schijven, MP},
  journal={Surgical endoscopy},
  volume={23},
  number={6},
  pages={1180--1190},
  year={2009},
  publisher={Springer}
}

@inproceedings{mullins2005haptic,
  title={Haptic handwriting aid for training and rehabilitation},
  author={Mullins, James and Mawson, Christopher and Nahavandi, Saeid},
  booktitle={Systems, Man and Cybernetics, 2005 IEEE International Conference on},
  volume={3},
  pages={2690--2694},
  year={2005},
  organization={IEEE}
}

@inproceedings{mullins2004soft,
  title={Soft tissue modelling for haptic rendering in virtual environments},
  author={Mullins, James and Trinh, Hieu and Nahavandi, Saeid},
  booktitle={Mechatronics 2004: 9th, Ankara, 30 Aug-1 Sept 2004: conference proceedings},
  pages={693--698},
  year={2004},
  organization={Atilim University}
}

@inproceedings{loureiro2001using,
  title={Using haptics technology to deliver motivational therapies in stroke patients: Concepts and initial pilot studies},
  author={Loureiro, Rui and Amirabdollahian, Farshid and Coote, Susan and Stokes, Emma and Harwin, William},
  booktitle={Proceedings of EuroHaptics},
  volume={2001},
  pages={6},
  year={2001}
}

@article{schmidt2005hapticwalker,
  title={HapticWalker---a novel haptic foot device},
  author={Schmidt, Henning and Hesse, Stefan and Bernhardt, Rolf and Kr{\"u}ger, J{\"o}rg},
  journal={ACM Transactions on Applied Perception (TAP)},
  volume={2},
  number={2},
  pages={166--180},
  year={2005},
  publisher={ACM}
}

@article{rajanna2016kinohaptics,
  title={KinoHaptics: An automated, wearable, Haptic assisted, physio-therapeutic system for post-surgery rehabilitation and self-care},
  author={Rajanna, Vijay and Vo, Patrick and Barth, Jerry and Mjelde, Matthew and Grey, Trevor and Oduola, Cassandra and Hammond, Tracy},
  journal={Journal of medical systems},
  volume={40},
  number={3},
  pages={60},
  year={2016},
  publisher={Springer}
}

@inproceedings{mihelj2008henrie,
  title={HEnRiE-Haptic environment for reaching and grasping exercise},
  author={Mihelj, Matjaz and Podobnik, Janez and Munih, Marko},
  booktitle={Biomedical Robotics and Biomechatronics, 2008. BioRob 2008. 2nd IEEE RAS \& EMBS International Conference on},
  pages={907--912},
  year={2008},
  organization={IEEE}
}

@book{merzouki2012intelligent,
  title={Intelligent mechatronic systems: modeling, control and diagnosis},
  author={Merzouki, Rochdi and Samantaray, Arun Kumar and Pathak, Pushparaj Mani and Bouamama, Belkacem Ould},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@misc{electromagnets,
  title={electromagnets},
  author={Unknown},
  year={Unknown},
  publisher={Museum of Science},
  howpublished = {\url{http://www.ece.neu.edu/fac-ece/nian/mom/electromagnets.html}},
  note = {Accessed: 2018-27-02}
}

@misc{electromagnet_wiki,
  title={Electromagnet},
  author={Unknown},
  year={Unknown},
  publisher={Wikipedia},
  howpublished = {\url{https://en.wikipedia.org/wiki/Electromagnet}},
  note = {Accessed: 2018-27-02}
}

@phdthesis{lam2012model,
  title={A model predictive approach to optimal path-following and contouring control},
  author={Lam, Denise},
  year={2012}
}


@article{cominos2002pid,
  title={PID controllers: recent tuning methods and design to specification},
  author={Cominos, P and Munro, N},
  journal={IEE Proceedings-Control Theory and Applications},
  volume={149},
  number={1},
  pages={46--53},
  year={2002},
  publisher={IET}
}

@book{aastrom1995pid,
  title={PID controllers: theory, design, and tuning},
  author={{\AA}str{\"o}m, Karl Johan and H{\"a}gglund, Tore},
  volume={2},
  year={1995},
  publisher={Instrument society of America Research Triangle Park, NC}
}

@article{erkorkmaz2001high,
  title={High speed CNC system design. Part III: high speed tracking and contouring control of feed drives},
  author={Erkorkmaz, Kaan and Altintas, Yusuf},
  journal={International Journal of Machine Tools and Manufacture},
  volume={41},
  number={11},
  pages={1637--1658},
  year={2001},
  publisher={Elsevier}
}

@phdthesis{ko2003high,
  title={High-speed and high-precision feedforward control of contouring machine tools},
  author={Ko, RC},
  year={2003},
  school={Ph. D. dissertation, University of Melbourne}
}

@article{dahunsi2010system,
  title={System identification and neural network based PID control of servo-hydraulic vehicle suspension system},
  author={Dahunsi, OA and Pedro, JO and Nyandoro, OT},
  journal={SAIEE Africa Research Journal},
  volume={101},
  number={3},
  pages={93--105},
  year={2010}
}

@article{koren1980cross,
  title={Cross-coupled biaxial computer control for manufacturing systems},
  author={Koren, Yoram},
  journal={Journal of Dynamic Systems, Measurement, and Control},
  volume={102},
  number={4},
  pages={265--272},
  year={1980},
  publisher={American Society of Mechanical Engineers}
}

@article{koren1992advanced,
  title={Advanced controllers for feed drives},
  author={Koren, Y and Lo, Ch-Ch},
  journal={CIRP Annals-Manufacturing Technology},
  volume={41},
  number={2},
  pages={689--698},
  year={1992},
  publisher={Elsevier}
}

@article{qin2003survey,
  title={A survey of industrial model predictive control technology},
  author={Qin, S Joe and Badgwell, Thomas A},
  journal={Control engineering practice},
  volume={11},
  number={7},
  pages={733--764},
  year={2003},
  publisher={Elsevier}
}

@article{morari1999model,
  title={Model predictive control: past, present and future},
  author={Morari, Manfred and Lee, Jay H},
  journal={Computers \& Chemical Engineering},
  volume={23},
  number={4-5},
  pages={667--682},
  year={1999},
  publisher={Elsevier}
}

@book{wang2009model,
  title={Model predictive control system design and implementation using MATLAB{\textregistered}},
  author={Wang, Liuping},
  year={2009},
  publisher={Springer Science \& Business Media}
}

@book{meunier2010finite,
  title={The finite element method for electromagnetic modeling},
  author={Meunier, G{\'e}rard},
  volume={33},
  year={2010},
  publisher={John Wiley \& Sons}
}

@article{liniger2015optimization,
  title={Optimization-based autonomous racing of 1: 43 scale RC cars},
  author={Liniger, Alexander and Domahidi, Alexander and Morari, Manfred},
  journal={Optimal Control Applications and Methods},
  volume={36},
  number={5},
  pages={628--647},
  year={2015},
  publisher={Wiley Online Library}
}

@inproceedings{lam2010model,
  title={Model predictive contouring control},
  author={Lam, Denise and Manzie, Chris and Good, Malcolm},
  booktitle={Decision and Control (CDC), 2010 49th IEEE Conference on},
  pages={6137--6142},
  year={2010},
  organization={IEEE}
}
@article{erkorkmaz2005quintic,
  title={Quintic spline interpolation with minimal feed fluctuation},
  author={Erkorkmaz, Kaan and Altintas, Yusuf},
  journal={Journal of Manufacturing Science and Engineering},
  volume={127},
  number={2},
  pages={339--349},
  year={2005},
  publisher={American Society of Mechanical Engineers}
}

@article{langhorne2009motor,
  title={Motor recovery after stroke: a systematic review},
  author={Langhorne, Peter and Coupar, Fiona and Pollock, Alex},
  journal={The Lancet Neurology},
  volume={8},
  number={8},
  pages={741--754},
  year={2009},
  publisher={Elsevier}
}

@article{langhammer2000bobath,
  title={Bobath or motor relearning programme? A comparison of two different approaches of physiotherapy in stroke rehabilitation: a randomized controlled study},
  author={Langhammer, Birgitta and Stanghelle, Johan K},
  journal={Clinical rehabilitation},
  volume={14},
  number={4},
  pages={361--369},
  year={2000},
  publisher={SAGE Publications Sage CA: Thousand Oaks, CA}
}

@article{french2007repetitive,
  title={Repetitive task training for improving functional ability after stroke},
  author={French, Beverley and Thomas, Lois H and Leathley, Michael J and Sutton, Christopher J and McAdam, Joanna and Forster, Anne and Langhorne, Peter and Price, CI and Walker, Andrew and Watkins, Caroline L},
  journal={Cochrane Database Syst Rev},
  volume={4},
  number={4},
  year={2007},
  publisher={Wiley Online Library}
}

@article{warlow2008stroke,
  title={Stroke: practical management},
  author={Warlow, Charles and Van Gijn, Jan and Dennis, Martin S and Wardlaw, Joanna M and Sandercock, Peter AG and Rinkel, Gabriel and Langhorne, Peter},
  year={2008},
  publisher={Blackwell publishing Oxford}
}

@article{duncan1983reliability,
  title={Reliability of the Fugl-Meyer assessment of sensorimotor recovery following cerebrovascular accident},
  author={Duncan, Pamela W and Propst, Martha and Nelson, Steven G},
  journal={Physical therapy},
  volume={63},
  number={10},
  pages={1606--1610},
  year={1983},
  publisher={Oxford University Press}
}

@article{masiero2007robotic,
  title={Robotic-assisted rehabilitation of the upper limb after acute stroke},
  author={Masiero, Stefano and Celia, Andrea and Rosati, Giulio and Armani, Mario},
  journal={Archives of physical medicine and rehabilitation},
  volume={88},
  number={2},
  pages={142--149},
  year={2007},
  publisher={Elsevier}
}

@article{kahn2006robot,
  title={Robot-assisted reaching exercise promotes arm movement recovery in chronic hemiparetic stroke: a randomized controlled pilot study},
  author={Kahn, Leonard E and Zygman, Michele L and Rymer, W Zev and Reinkensmeyer, David J},
  journal={Journal of neuroengineering and rehabilitation},
  volume={3},
  number={1},
  pages={12},
  year={2006},
  publisher={BioMed Central}
}

@article{lum2002robot,
  title={Robot-assisted movement training compared with conventional therapy techniques for the rehabilitation of upper-limb motor function after stroke},
  author={Lum, Peter S and Burgar, Charles G and Shor, Peggy C and Majmundar, Matra and Van der Loos, Machiel},
  journal={Archives of physical medicine and rehabilitation},
  volume={83},
  number={7},
  pages={952--959},
  year={2002},
  publisher={Elsevier}
}

@article{nageli2017real,
  title={Real-time planning for automated multi-view drone cinematography},
  author={N{\"a}geli, Tobias and Meier, Lukas and Domahidi, Alexander and Alonso-Mora, Javier and Hilliges, Otmar},
  journal={ACM Transactions on Graphics (TOG)},
  volume={36},
  number={4},
  pages={132},
  year={2017},
  publisher={ACM}
}

@book{schmidt2018motor,
  title={Motor Control and Learning, 6E},
  author={Schmidt, Richard A and Lee, Tim and Winstein, Carolee and Wulf, Gabriele and Zelaznik, Howard},
  year={2018},
  publisher={Human kinetics}
}

@article{adams1971closed,
  title={Closed-loop theory and long-term retention.},
  author={Adams, Jack A and Marshall, Philip H and Bray, Norman W},
  year={1971},
  publisher={American Psychological Association}
}

@article{schmidt1975schema,
  title={A schema theory of discrete motor skill learning.},
  author={Schmidt, Richard A},
  journal={Psychological review},
  volume={82},
  number={4},
  pages={225},
  year={1975},
  publisher={American Psychological Association}
}

@book{rosenbaum2009human,
  title={Human motor control},
  author={Rosenbaum, David A},
  year={2009},
  publisher={Academic press}
}

@article{shusterman2011muscle,
  title={Muscle memory and the somaesthetic pathologies of everyday life},
  author={Shusterman, Richard},
  journal={Human Movement},
  volume={12},
  number={1},
  pages={4--15},
  year={2011},
  publisher={Versita}
}

@article{wolpert1995arm,
  title={Are arm trajectories planned in kinematic or dynamic coordinates? An adaptation study},
  author={Wolpert, Daniel M and Ghahramani, Zoubin and Jordan, Michael I},
  journal={Experimental brain research},
  volume={103},
  number={3},
  pages={460--470},
  year={1995},
  publisher={Springer}
}

@article{sigrist2013augmented,
  title={Augmented visual, auditory, haptic, and multimodal feedback in motor learning: a review},
  author={Sigrist, Roland and Rauter, Georg and Riener, Robert and Wolf, Peter},
  journal={Psychonomic bulletin \& review},
  volume={20},
  number={1},
  pages={21--53},
  year={2013},
  publisher={Springer}
}

@article{hale2004deriving,
  title={Deriving haptic design guidelines from human physiological, psychophysical, and neurological foundations},
  author={Hale, Kelly S and Stanney, Kay M},
  journal={IEEE Computer Graphics and Applications},
  volume={24},
  number={2},
  pages={33--39},
  year={2004},
  publisher={IEEE}
}

@article{scheidt2000persistence,
  title={Persistence of motor adaptation during constrained, multi-joint, arm movements},
  author={Scheidt, Robert A and Reinkensmeyer, David J and Conditt, Michael A and Rymer, W Zev and Mussa-Ivaldi, Ferdinando A},
  journal={Journal of Neurophysiology},
  volume={84},
  number={2},
  pages={853--862},
  year={2000},
  publisher={Am Physiological Soc}
}

@article{Marchal2008motor,
author = { Laura Marchal   Crespo  and  David J.   Reinkensmeyer },
title = {Haptic Guidance Can Enhance Motor Learning of a Steering Task},
journal = {Journal of Motor Behavior},
volume = {40},
number = {6},
pages = {545-557},
year  = {2008},
publisher = {Routledge},
doi = {10.3200/JMBR.40.6.545-557},
URL = { 
        https://doi.org/10.3200/JMBR.40.6.545-557
    
},
}

@inproceedings{accot1997beyond,
  title={Beyond Fitts' law: models for trajectory-based HCI tasks},
  author={Accot, Johnny and Zhai, Shumin},
  booktitle={Proceedings of the ACM SIGCHI Conference on Human factors in computing systems},
  pages={295--302},
  year={1997},
  organization={ACM}
}


@article{marchal2010effect,
  title={The effect of haptic guidance, aging, and initial skill level on motor learning of a steering task},
  author={Marchal-Crespo, Laura and McHughen, Stephanie and Cramer, Steven C and Reinkensmeyer, David J},
  journal={Experimental brain research},
  volume={201},
  number={2},
  pages={209--220},
  year={2010},
  publisher={Springer}
}

@article{hidler2009multicenter,
  title={Multicenter randomized clinical trial evaluating the effectiveness of the Lokomat in subacute stroke},
  author={Hidler, Joseph and Nichols, Diane and Pelliccio, Marlena and Brady, Kathy and Campbell, Donielle D and Kahn, Jennifer H and Hornby, T George},
  journal={Neurorehabilitation and neural repair},
  volume={23},
  number={1},
  pages={5--13},
  year={2009},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@article{husemann2007effects,
  title={Effects of locomotion training with assistance of a robot-driven gait orthosis in hemiparetic patients after stroke: a randomized controlled pilot study},
  author={Husemann, Britta and M{\"u}ller, Friedemann and Krewer, Carmen and Heller, Silke and Koenig, Eberhardt},
  journal={Stroke},
  volume={38},
  number={2},
  pages={349--354},
  year={2007},
  publisher={Am Heart Assoc}
}

@misc{hyst,
  title={PID controller},
  author={Nave, Carl},
  year={2017},
  publisher={hyperphysics},
  howpublished = {\url{http://hyperphysics.phy-astr.gsu.edu/hbase/Solids/hyst.html}},
  note = {Accessed: 2018-14-03}
}

@inproceedings{Naegeli:2017:MultiDroneCine,
	author = {N{\"a}geli, Tobias and Meier, Lukas and Domahidi, Alexander and Alonso-Mora, Javier and Hilliges, Otmar},
	title = {Real-time Planning for Automated Multi-View Drone Cinematography},
	journal = {ACM Transactions on Graphics (Proceedings of ACM SIGGRAPH)},
	year = {2017},
	location = {Los Angeles, USA},
}

@mics{forcespro,
title={FORCES Pro: code generation for embedded optimization.},
author={Domahidi, Alexander and Jerez, Juan},
year={2016},
howpublished = {\url{https://www.embotech.com/FORCES-Pro}}
}
@inproceedings{frisoli2005new,
  title={A new force-feedback arm exoskeleton for haptic interaction in virtual environments},
  author={Frisoli, Antonio and Rocchi, Fabrizio and Marcheschi, Simone and Dettori, Andrea and Salsedo, Fabio and Bergamasco, Massimo},
  booktitle={Eurohaptics Conference, 2005 and Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems, 2005. World Haptics 2005. First Joint},
  pages={195--201},
  year={2005},
  organization={IEEE}
}
@article{ali2012too,
  title={Too much of a good thing: random practice scheduling and self-control of feedback lead to unique but not additive learning benefits},
  author={Ali, Asif and Fawver, Bradley and Fairbrother, Jeffrey T and Janelle, Christopher M},
  journal={Frontiers in psychology},
  volume={3},
  pages={503},
  year={2012},
  publisher={Frontiers}
}

@article{kawato1999internal,
  title={Internal models for motor control and trajectory planning},
  author={Kawato, Mitsuo},
  journal={Current opinion in neurobiology},
  volume={9},
  number={6},
  pages={718--727},
  year={1999},
  publisher={Elsevier}
}




@article{limpaecher2013real,
  title={Real-time drawing assistance through crowdsourcing},
  author={Limpaecher, Alex and Feltman, Nicolas and Treuille, Adrien and Cohen, Michael},
  journal={ACM Transactions on Graphics (TOG)},
  volume={32},
  number={4},
  pages={54},
  year={2013},
  publisher={ACM}
}

@article{favreau2016fidelity,
  title={Fidelity vs. simplicity: a global approach to line drawing vectorization},
  author={Favreau, Jean-Dominique and Lafarge, Florent and Bousseau, Adrien},
  journal={ACM Transactions on Graphics (TOG)},
  volume={35},
  number={4},
  pages={120},
  year={2016},
  publisher={ACM}
}

@inproceedings{lee2011shadowdraw,
  title={Shadowdraw: real-time user guidance for freehand drawing},
  author={Lee, Yong Jae and Zitnick, C Lawrence and Cohen, Michael F},
  booktitle={ACM Transactions on Graphics (TOG)},
  volume={30},
  number={4},
  pages={27},
  year={2011},
  organization={ACM}
}

@article{liu2018strokeaggregator,
  title={StrokeAggregator: consolidating raw sketches into artist-intended curve drawings},
  author={Liu, Chenxi and Rosales, Enrique and Sheffer, Alla},
  journal={ACM Transactions on Graphics (TOG)},
  volume={37},
  number={4},
  pages={97},
  year={2018},
  publisher={ACM}
}

@article{simo2016learning,
  title={Learning to simplify: fully convolutional networks for rough sketch cleanup},
  author={Simo-Serra, Edgar and Iizuka, Satoshi and Sasaki, Kazuma and Ishikawa, Hiroshi},
  journal={ACM Transactions on Graphics (TOG)},
  volume={35},
  number={4},
  pages={121},
  year={2016},
  publisher={ACM}
}


@article{simo2018real,
  title={Real-time data-driven interactive rough sketch inking},
  author={Simo-Serra, Edgar and Iizuka, Satoshi and Ishikawa, Hiroshi},
  journal={ACM Transactions on Graphics (TOG)},
  volume={37},
  number={4},
  pages={98},
  year={2018},
  publisher={ACM}
}


@article{simo2018mastering,
  title={Mastering sketching: adversarial augmentation for structured prediction},
  author={Simo-Serra, Edgar and Iizuka, Satoshi and Ishikawa, Hiroshi},
  journal={ACM Transactions on Graphics (TOG)},
  volume={37},
  number={1},
  pages={11},
  year={2018},
  publisher={ACM}
}

@book{gibbs2011advanced,
  title={Advanced Kalman filtering, least-squares and modeling: a practical handbook},
  author={Gibbs, Bruce P},
  year={2011},
  publisher={John Wiley \& Sons}
}

@book{rockafellar2009variational,
  title={Variational analysis},
  author={Rockafellar, R Tyrrell and Wets, Roger J-B},
  volume={317},
  year={2009},
  publisher={Springer Science \& Business Media}
}


@article{su2014ez,
  title={EZ-sketching: three-level optimization for error-tolerant image tracing},
  author={Su, Qingkun and Li, Wing Ho Andy and Wang, Jue and Fu, Hongbo},
  journal={ACM Transactions on Graphics},
  volume={33},
  number={4},
  year={2014},
  publisher={ACM Special Interest Group}
}

@article{hilaire2006robust,
  title={Robust and accurate vectorization of line drawings},
  author={Hilaire, Xavier and Tombre, Karl},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={28},
  number={6},
  pages={890--904},
  year={2006},
  publisher={IEEE}
}

@article{xing2015autocomplete,
  title={Autocomplete hand-drawn animations},
  author={Xing, Jun and Wei, Li-Yi and Shiratori, Takaaki and Yatani, Koji},
  journal={ACM Transactions on Graphics (TOG)},
  volume={34},
  number={6},
  pages={169},
  year={2015},
  publisher={ACM}
}

@inproceedings{peng2015d,
  title={D-Coil: A Hands-on Approach to Digital 3D Models Design},
  author={Peng, Huaishu and Zoran, Amit and Guimbreti{\`e}re, Fran{\c{c}}ois V},
  booktitle={Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
  pages={1807--1815},
  year={2015},
  organization={ACM}
}


@article{kolmogorov1933sulla,
  title={Sulla determinazione empirica di una lgge di distribuzione},
  author={Kolmogorov, Andrey},
  journal={Inst. Ital. Attuari, Giorn.},
  volume={4},
  pages={83--91},
  year={1933}
}

@article{savitzky1964smoothing,
  title={Smoothing and differentiation of data by simplified least squares procedures.},
  author={Savitzky, Abraham and Golay, Marcel JE},
  journal={Analytical chemistry},
  volume={36},
  number={8},
  pages={1627--1639},
  year={1964},
  publisher={ACS Publications}
}


@book{loomis1939fun,
  title={Fun with a Pencil},
  author={Loomis, Andrew},
  year={1939},
  publisher={Viking Press}
}

@article{zoran2014wise,
  title={The wise chisel: The rise of the smart handheld tool},
  author={Zoran, Amit and Shilkrot, Roy and Goyal, Pragun and Maes, Pattie and Paradiso, Joseph A},
  journal={IEEE Pervasive Computing},
  volume={13},
  number={3},
  pages={48--57},
  year={2014},
  publisher={IEEE}
}
@inproceedings{zoran2013freed,
  title={FreeD: a freehand digital sculpting tool},
  author={Zoran, Amit and Paradiso, Joseph A},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={2613--2616},
  year={2013},
  organization={ACM}
}

@inproceedings{portillo2005haptic,
  title={Haptic desktop for assisted handwriting and drawing},
  author={Portillo, O and Avizzano, Carlo Alberto and Raspolli, Mirko and Bergamasco, Massimo},
  booktitle={ROMAN 2005. IEEE International Workshop on Robot and Human Interactive Communication, 2005.},
  pages={512--517},
  year={2005},
  organization={IEEE}
}

@inproceedings{yang2008validating,
  title={Validating the performance of haptic motor skill training},
  author={Yang, Xing-Dong and Bischof, Walter F and Boulanger, Pierre},
  booktitle={2008 Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems},
  pages={129--135},
  year={2008},
  organization={IEEE}
}


%%%% Biblio magtics
@inproceedings{Jang2016,
 author = {Jang, Sungjune and Kim, Lawrence H. and Tanner, Kesler and Ishii, Hiroshi and Follmer, Sean},
 title = {{Haptic Edge Display for Mobile Tactile Interaction}},
 booktitle = {Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '16},
 year = {2016},
 isbn = {978-1-4503-3362-7},
 location = {Santa Clara, California, USA},
 pages = {3706--3716},
 numpages = {11},
 url = {http://doi.acm.org/10.1145/2858036.2858264},
 doi = {10.1145/2858036.2858264},
 acmid = {2858264},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {dynamic affordance, mobile haptics, tactile display}
}

@inproceedings{Benko2016,
 author = {Benko, Hrvoje and Holz, Christian and Sinclair, Mike and Ofek, Eyal},
 title = {{NormalTouch and TextureTouch: High-fidelity 3D Haptic Shape Rendering on Handheld Virtual Reality Controllers}},
 booktitle = {Proceedings of the 29th Annual Symposium on User Interface Software and Technology},
 series = {UIST '16},
 year = {2016},
 isbn = {978-1-4503-4189-9},
 location = {Tokyo, Japan},
 pages = {717--728},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2984511.2984526},
 doi = {10.1145/2984511.2984526},
 acmid = {2984526},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {controller design, haptics, tactile display, virtual reality}
 }

 @inproceedings{Kim2016,
 author = {Kim, Hwan and Kim, Minhwan and Lee, Woohun},
 title = {{HapThimble: A Wearable Haptic Device Towards Usable Virtual Touch Screen}},
 booktitle = {Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '16},
 year = {2016},
 isbn = {978-1-4503-3362-7},
 location = {Santa Clara, California, USA},
 pages = {3694--3705},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2858036.2858196},
 doi = {10.1145/2858036.2858196},
 acmid = {2858196},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {direct-touch interaction, haptic feedback without haptic constraint, virtual touch screen, wearable haptic device}
} 

@inproceedings{Choi2016,
 author = {Choi, Inrak and Follmer, Sean},
 title = {{Wolverine: A Wearable Haptic Interface for Grasping in VR}},
 booktitle = {Proceedings of the 29th Annual Symposium on User Interface Software and Technology},
 series = {UIST '16 Adjunct},
 year = {2016},
 isbn = {978-1-4503-4531-6},
 location = {Tokyo, Japan},
 pages = {117--119},
 numpages = {3},
 url = {http://doi.acm.org/10.1145/2984751.2985725},
 doi = {10.1145/2984751.2985725},
 acmid = {2985725},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {force feedback, virtual reality, wearable haptic interfaces}
} 

@inproceedings{Machida2015,
 author = {Machida, Taiga and Dim, Nem Khan and Ren, Xiangshi},
 title = {{Suitable Body Parts for Vibration Feedback in Walking Navigation Systems}},
 booktitle = {Proceedings of the Third International Symposium of Chinese CHI},
 series = {Chinese CHI '15},
 year = {2015},
 isbn = {978-1-4503-3464-8},
 location = {Seoul, Republic of Korea},
 pages = {32--36},
 numpages = {5},
 url = {http://doi.acm.org/10.1145/2739999.2740004},
 doi = {10.1145/2739999.2740004},
 acmid = {2740004},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Map navigation systems, vibration feedback}
}

@misc{Vivosmart,
	author = {Garmin},
	title = {{Vivosmart\textsuperscript{\textregistered}}},
	howpublished = {\url{https://buy.garmin.com/en-US/US/p/154886}},
	note = {Last accessed: 07.03.2017}
}

@misc{Cybergrasp,
	author = {{CyberGlove Systems Inc.}},
	title = {{CyberGrasp Glove}},
	howpublished = {\url{http://www.cyberglovesystems.com/cybergrasp}},
	note = {Last accessed: 12.03.2017}
}

@misc{Cybertouch,
	author = {{CyberGlove Systems Inc.}},
	title = {{CyberTouch Glove}},
	howpublished = {\url{http://www.cyberglovesystems.com/cybertouch}},
	note = {Last accessed: 18.03.2017}
}

@misc{Gloveone,
	author = {{NeuroDigital Technologies}},
	title = {{Gloveone Glove}},
	howpublished = {\url{https://www.neurodigital.es/gloveone/}},
	note = {Last accessed: 29.03.2017}
}

@misc{HTCVive,
	author = {{HTC Corp.}},
	title = {{HTC Vive}},
	howpublished = {\url{https://www.vive.com/eu/}},
	note = {Last accessed: 29.03.2017}
}

@inproceedings{Gu2016,
 author = {Gu, Xiaochi and Zhang, Yifei and Sun, Weize and Bian, Yuanzhe and Zhou, Dao and Kristensson, Per Ola},
 title = {{Dexmo: An Inexpensive and Lightweight Mechanical Exoskeleton for Motion Capture and Force Feedback in VR}},
 booktitle = {Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '16},
 year = {2016},
 isbn = {978-1-4503-3362-7},
 location = {Santa Clara, California, USA},
 pages = {1991--1995},
 numpages = {5},
 url = {http://doi.acm.org/10.1145/2858036.2858487},
 doi = {10.1145/2858036.2858487},
 acmid = {2858487},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {exoskeleton, force feedback, motion capture, virtual reality}
} 

@misc{AthleteSurvey,
	author = {{Athlete IQ}},
	title = {{ Voice of the Athlete Survey. Wearable Devices In the Active Lifestyle Market}},
	howpublished = {\url{http://www.sporttechie.com/wp-content/uploads/2016/02/Wearable-Device-Survey-Results-2.pdf}},
	note = {Last accessed: 10.03.2017}
}

@article{Hayward2004,
	author = {Hayward, Vincent and Astley, Oliver R. and Cruz‐Hernandez, Manuel and Grant, Danny and Robles‐De‐La‐Torre, Gabriel},
	title = {{Haptic Interfaces and Devices}},
	journal = {Sensor Review},
	volume = {24},
	number = {1},
	pages = {16--29},
	year = {2004},
	doi = {10.1108/02602280410515770}
}

@article{Niu2012,
author = {Niu, Xiaofan and Yang, Xinguo and Brochu, Paul and Stoyanov, Hristiyan and Yun, Sungryul and Yu, Zhibin and Pei, Qibing},
doi = {10.1002/adma.201202876},
journal = {Advanced Materials},
keywords = {Braille display,actuation,bistable electroactive polymers,interpenetrating polymer networks,polymer swelling},
month = {dec},
number = {48},
pages = {6513--6519},
pmid = {22987622},
title = {{Bistable Large-Strain Actuation of Interpenetrating Polymer Networks}},
url = {http://doi.wiley.com/10.1002/adma.201202876},
volume = {24},
year = {2012}
}

@inproceedings{Szabo2016,
author = {Szabo, Zoltan and Enikov, Eniko T},
doi = {10.1007/978-3-319-41267-2_8},
isbn = {978-3-319-41267-2},
pages = {53--60},
publisher = {Springer International Publishing},
title = {{Electromagnetic Microactuator-Array Based Virtual Tactile Display}},
booktitle = {Computers Helping People with Special Needs: 15th International Conference, ICCHP 2016},
year = {2016}
}

@article {Streque2012,
	author = {Streque, J., Talbi, a, Pernod, P., Preobrazhensky, V.},
    title = {{Pulse-driven Magnetostatic Micro-actuator Array Based on Ultrasoft Elastomeric Membranes for Active Surface Applications}},
    journal = {Journal of Micromechanics and Microengineering},
    volume = {22},
	number = {9},
	pages = {95020},
	year = {2012},
	doi = {10.1088/0960-1317/22/9/095020}
}


@inproceedings{Wu2012,
author = {Wu, You and Schmidt, Lara and Parker, Matthew and Strong, John and Bruns, Michael and Ramani, Viniyak Karthik},
number = {45011},
pages = {1481--1490},
title = {{ACTIVE-Hand: Automatic Configurable Tactile Interaction in Virtual Environment}},
url = {http://dx.doi.org/10.1115/DETC2012-71326},
year = {2012}
}


@inproceedings{Strasnick2016,
	author = {Evan Strasnick and Sean Follmer},
	title = {{Applications of Switchable Permanent Magnetic Actuators in Shape Change and Tactile Display}},
	booktitle = {n Proceedings of the 29th Annual Symposium on User Interface Software and Technology (UIST '16 Adjunct)},
	series = {UIST '16},
	year = {2016},
	doi = {10.1145/2984751.2985728},
    }
    
@inproceedings{Poupyrev2003,
	author = {Poupyrev, Ivan and Maruyama, Shigeaki},
	title = {{Tactile Interfaces for Small Touch Screens}},
	booktitle = {Proceedings of the 16th Annual ACM Symposium on User Interface Software and Technology},
	series = {UIST '03},
	year = {2003},
	isbn = {1-58113-636-6},
	location = {Vancouver, Canada},
	pages = {217--220},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/964696.964721},
	doi = {10.1145/964696.964721},
	acmid = {964721},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {mobile computers, tactile feedback, touch screen}
}

@inproceedings{Poupyrev2002,
	author = {Poupyrev, Ivan and Maruyama, Shigeaki and Rekimoto, Jun},
	title = {{Ambient Touch: Designing Tactile Interfaces for Handheld Devices}},
	booktitle = {Proceedings of the 15th Annual ACM Symposium on User Interface Software and Technology},
	series = {UIST '02},
	year = {2002},
	isbn = {1-58113-488-6},
	location = {Paris, France},
	pages = {51--60},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/571985.571993},
	doi = {10.1145/571985.571993},
	acmid = {571993},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {mobile devices and interfaces, tactile feedback}
} 

@inproceedings{Bouzit2002,
	author = {Bouzit, Mourad and Popescu, George and Burdea, Grigore and Boian, Rares},
	title = {{The Rutgers Master II-ND Force Feedback Glove}},
	booktitle = {Proceedings of the 10th Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems},
	series = {HAPTICS '02},
	year = {2002},
	isbn = {0-7695-1489-8},
	pages = {145},
	url = {http://dl.acm.org/citation.cfm?id=795682.797508},
	acmid = {797508},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Haptic glove, control, CyberGrasp, actuators, calibration, kinematics model, sensors, RMII, RMII-ND}
} 

@inproceedings{VanDerLinde2002,
	author = {Van Der Linde, R. Q. and Lammertse, P. and Frederiksen E. and Ruiter B.},
	title = {The {HapticMaster}, a New Highperformance Haptic Interface},
	booktitle = {Proceedings of Eurohaptics 2002},
	year = {2002}
} 



@article{Prattichizzo2013,
 author = {Prattichizzo, Domenico and Chinello, Francesco and Pacchierotti, Claudio and Malvezzi, Monica},
 title = {{Towards Wearability in Fingertip Haptics: a 3-DoF Wearable Device for Cutaneous Force Feedback}},
 journal = {EEE Trans. Haptics},
 volume = {6},
 number = {4},
 month = {Oct},
 year = {2013},
 issn = {1939-1412},
 pages = {506--516},
 numpages = {11},
 url = {http://dx.doi.org/10.1109/TOH.2013.53},
 doi = {10.1109/TOH.2013.53},
 acmid = {2574419},
 publisher = {IEEE Computer Society Press},
 address = {Los Alamitos, CA, USA}, 
 keywords = {Haptic interfaces,Wearable computers,Mobile communication,Fingers,Load modeling,portable computers,Haptic interfaces,force feedback,wearable computers}
}

@article{Krusteva2015,
 title={{Marionette: a Multi-Finger Tilt Feedback Device for Curvatures and Haptic Images Perception}},
 author = {Krusteva, Diana and Sahoo, Deepak and Asier, Marzo and Subramanian, Sriram and Coyle, David},
 booktitle = {Proceedings of the 2015 CHI Conference on Human Factors in Computing Systems},
 series = {CHI EA '15},
 year = {2015},
 isbn = {},
 location = {Seoul, South Korea},
 pages = {1229-1234},
 numpages = {5},
 url = {http://dx.doi.org/10.1145/2702613.2732729},
 doi = {10.1145/2702613.2732729},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Haptic perception; Touch; Curvature discrimination; Multi-fringe}
}


@inproceedings{Iwata2001,
 author = {Iwata, Hiroo and Yano, Hiroaki and Nakaizumi, Fumitaka and Kawamura, Ryo},
 title = {{Project FEELEX: Adding Haptic Surface to Graphics}},
 booktitle = {Proceedings of the 28th Annual Conference on Computer Graphics and Interactive Techniques},
 series = {SIGGRAPH '01},
 year = {2001},
 isbn = {1-58113-374-X},
 pages = {469--476},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/383259.383314},
 doi = {10.1145/383259.383314},
 acmid = {383314},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {actuator array, deformable screen, haptics, interactive graphics}
} 

@inproceedings{Carcedo2016,
 author = {Carcedo, Marta G. and Chua, Soon Hau and Perrault, Simon and Wozniak, Pawe\l and Joshi, Raj and Obaid, Mohammad and Fjeld, Morten and Zhao, Shengdong},
 title = {{HaptiColor: Interpolating Color Information As Haptic Feedback to Assist the Colorblind}},
 booktitle = {Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '16},
 year = {2016},
 isbn = {978-1-4503-3362-7},
 location = {Santa Clara, California, USA},
 pages = {3572--3583},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2858036.2858220},
 doi = {10.1145/2858036.2858220},
 acmid = {2858220},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {color blindness, spatiotemporal vibrotactile pattern, vibration, wearable computing, wristband}
} 

@article{Kyung2009,
 author = {Kyung, Ki-Uk and Lee, Jun-Young},
 title = {{Ubi-Pen: A Haptic Interface with Texture and Vibrotactile Display}},
 journal = {IEEE Comput. Graph. Appl.},
 issue_date = {January/February 2009},
 volume = {29},
 number = {1},
 month = jan,
 year = {2009},
 issn = {0272-1716},
 pages = {56--64},
 numpages = {9},
 url = {http://dx.doi.org/10.1109/MCG.2009.17},
 doi = {10.1109/MCG.2009.17},
 acmid = {1669278},
 publisher = {IEEE Computer Society Press},
 address = {Los Alamitos, CA, USA}
} 

@inproceedings{Lee2004,
 author = {Lee, Johnny C. and Dietz, Paul H. and Leigh, Darren and Yerazunis, William S. and Hudson, Scott E.},
 title = {{Haptic Pen: A Tactile Feedback Stylus for Touch Screens}},
 booktitle = {Proceedings of the 17th Annual ACM Symposium on User Interface Software and Technology},
 series = {UIST '04},
 year = {2004},
 isbn = {1-58113-957-8},
 location = {Santa Fe, NM, USA},
 pages = {291--294},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/1029632.1029682},
 doi = {10.1145/1029632.1029682},
 acmid = {1029682},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {haptic, multiuser, stylus, tactile feedback, touch screen}
} 

@inproceedings{Rekimoto2013,
 author = {Rekimoto, Jun},
 title = {{Traxion: A Tactile Interaction Device with Virtual Force Sensation}},
 booktitle = {Proceedings of the 26th Annual ACM Symposium on User Interface Software and Technology},
 series = {UIST '13},
 year = {2013},
 isbn = {978-1-4503-2268-3},
 location = {St. Andrews, Scotland, United Kingdom},
 pages = {427--432},
 numpages = {6},
 url = {http://doi.acm.org/10.1145/2501988.2502044},
 doi = {10.1145/2501988.2502044},
 acmid = {2502044},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {illusion, input devices, tactile interactions},
} 

@inproceedings{Lee2015ThreeByThree,
 author = {Lee, Jaeyeon and Han, Jaehyun and Lee, Geehyuk},
 title = {{Investigating the Information Transfer Efficiency of a 3x3 Watch-back Tactile Display}},
 booktitle = {Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
 series = {CHI '15},
 year = {2015},
 isbn = {978-1-4503-3145-6},
 location = {Seoul, Republic of Korea},
 pages = {1229--1232},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/2702123.2702530},
 doi = {10.1145/2702123.2702530},
 acmid = {2702530},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {3x3 tactor array, information transfer efficiency, watch-back tactile display},
} 

@inproceedings{Gupta2016,
 author = {Gupta, Aakar and Pietrzak, Thomas and Roussel, Nicolas and Balakrishnan, Ravin},
 title = {{Direct Manipulation in Tactile Displays}},
 booktitle = {Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '16},
 year = {2016},
 isbn = {978-1-4503-3362-7},
 location = {Santa Clara, California, USA},
 pages = {3683--3693},
 numpages = {11},
 url = {http://doi.acm.org/10.1145/2858036.2858161},
 doi = {10.1145/2858036.2858161},
 acmid = {2858161},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {direct manipulation, tactile displays, wearables, wrist},
} 

@inproceedings{Lee2010BuzzWear,
 author = {Lee, Seungyon "Claire" and Starner, Thad},
 title = {{BuzzWear: Alert Perception in Wearable Tactile Displays on the Wrist}},
 booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
 series = {CHI '10},
 year = {2010},
 isbn = {978-1-60558-929-9},
 location = {Atlanta, Georgia, USA},
 pages = {433--442},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1753326.1753392},
 doi = {10.1145/1753326.1753392},
 acmid = {1753392},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {attention, tactile display, wearable computing},
} 

@inproceedings{Wellman1995,
    author = {Wellman, Parris  and Howe, Robert D.},
    booktitle = {Proceedings of the ASME Dynamic Systems and Control Division},
    citeulike-article-id = {6599148},
    keywords = {tactile, vr},
    pages = {713--718},
    posted-at = {2010-01-28 12:29:45},
    priority = {1},
    title = {{Towards Realistic Vibrotactile Display in Virtual Environments}},
    year = {1995}
}

@ARTICLE{Kontarinis96,
    author = {Dimitrios A. Kontarinis and Robert D. Howe},
    title = {{Tactile Display of Vibratory Information in Teleoperation and Virtual Environments}},
    journal = {Presence},
    year = {1996},
    volume = {4},
    pages = {387--402}
}

@phdthesis{Stamper1997,
    title    = {{A Three Degree Of Freedom Parallel Manipulator With Only Translational Degrees Of Freedom}},
    school   = {University of Maryland at College Park},
    author   = {Stamper, Richard E.},
    year     = {1997}
}

@phdthesis{Brady2010,
    title    = {{Tactile Arrays for Virtual Textures}},
    school   = {Exeter},
    author   = {Brady, Alan Christopher},
    year     = {2010}
}

@inproceedings{Summers2001,
 author = {Summers, Ian R. and Chanter,Craig M. and Southall, Anna L. and Brady, Alan C.},
 title = {{Results from a Tactile Array on the Fingertip}},
 booktitle = {Proceedings of Proceedings of Eurohaptics 2001},
 year = {2001}
} 

@inproceedings{Araujo2016,
 author = {Araujo, Bruno and Jota, Ricardo and Perumal, Varun and Yao, Jia Xian and Singh, Karan and Wigdor, Daniel},
 title = {{Snake Charmer: Physically Enabling Virtual Objects}},
 booktitle = {Proceedings of the TEI '16: Tenth International Conference on Tangible, Embedded, and Embodied Interaction},
 series = {TEI '16},
 year = {2016},
 isbn = {978-1-4503-3582-9},
 location = {Eindhoven, Netherlands},
 pages = {218--226},
 numpages = {9},
 url = {http://doi.acm.org/10.1145/2839462.2839484},
 doi = {10.1145/2839462.2839484},
 acmid = {2839484},
 publisher = {ACM},
 address = {New York, NY, USA}
} 

@inproceedings{Wang2016,
 author = {Wang, Qinglong and Ren, Xiangshi and Sun, Xiaoying},
 title = {{EV-pen: an Electrovibration Haptic Feedback Pen for Touchscreens}},
 booktitle = {SIGGRAPH ASIA 2016 Emerging Technologies},
 series = {SA '16},
 year = {2016},
 isbn = {978-1-4503-4539-2},
 location = {Macau},
 pages = {8:1--8:2},
 articleno = {8},
 numpages = {2},
 url = {http://doi.acm.org/10.1145/2988240.2988241},
 doi = {10.1145/2988240.2988241},
 acmid = {2988241},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {electrovibration, haptic feedback, pen, touch screen}
} 

@inproceedings{Takanaka2015,
 author = {Takanaka, Shun and Yano, Hiroaki and Iwata, Hiroo},
 title = {{Multitouch Haptic Interface with Movable Touch Screen}},
 booktitle = {SIGGRAPH Asia 2015 Haptic Media And Contents Design},
 series = {SA '15},
 year = {2015},
 isbn = {978-1-4503-3932-2},
 location = {Kobe, Japan},
 pages = {13:1--13:3},
 articleno = {13},
 numpages = {3},
 url = {http://doi.acm.org/10.1145/2818384.2818396},
 doi = {10.1145/2818384.2818396},
 acmid = {2818396},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {haptic interface, multitouch, shearing force, virtual reality}
} 

@inproceedings{Hoffman1998,
 author = {Hoffman, Hunter G.},
 title = {{Physically Touching Virtual Objects Using Tactile Augmentation Enhances the Realism of Virtual Environments}},
 booktitle = {Proceedings of the Virtual Reality Annual International Symposium},
 series = {VRAIS '98},
 year = {1998},
 isbn = {0-8186-8362-7},
 pages = {59},
 url = {http://dl.acm.org/citation.cfm?id=522258.836098},
 acmid = {836098},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA}
} 

@article{Hoshi2010,
 author = {Hoshi, Takayuki and Takahashi, Masafumi and Iwamoto, Takayuki and Shinoda, Hiroyuki},
 title = {{Noncontact Tactile Display Based on Radiation Pressure of Airborne Ultrasound}},
 journal = {EEE Trans. Haptics},
 issue_date = {July 2010},
 volume = {3},
 number = {3},
 month = jul,
 year = {2010},
 issn = {1939-1412},
 pages = {155--165},
 numpages = {11},
 url = {http://dx.doi.org/10.1109/TOH.2010.4},
 doi = {10.1109/TOH.2010.4},
 acmid = {1908041},
 publisher = {IEEE Computer Society Press},
 address = {Los Alamitos, CA, USA},
 keywords = {3D displays, Emerging technologies, Emerging technologies, haptic I/O, tactile displays, 3D displays, virtual reality., haptic I/O, tactile displays, virtual reality.}
} 

@inproceedings{Poupyrev2004,
 author = {Poupyrev, Ivan and Nashida, Tatsushi and Maruyama, Shigeaki and Rekimoto, Jun and Yamaji, Yasufumi},
 title = {{Lumen: Interactive Visual and Shape Display for Calm Computing}},
 booktitle = {ACM SIGGRAPH 2004 Emerging Technologies},
 series = {SIGGRAPH '04},
 year = {2004},
 isbn = {1-58113-896-2},
 location = {Los Angeles, California},
 pages = {17},
 url = {http://doi.acm.org/10.1145/1186155.1186173},
 doi = {10.1145/1186155.1186173},
 acmid = {1186173},
 publisher = {ACM},
 address = {New York, NY, USA}
} 

@inproceedings{Bau2010,
 author = {Bau, Olivier and Poupyrev, Ivan and Israr, Ali and Harrison, Chris},
 title = {{TeslaTouch: Electrovibration for Touch Surfaces}},
 booktitle = {Proceedings of the 23Nd Annual ACM Symposium on User Interface Software and Technology},
 series = {UIST '10},
 year = {2010},
 isbn = {978-1-4503-0271-5},
 location = {New York, New York, USA},
 pages = {283--292},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1866029.1866074},
 doi = {10.1145/1866029.1866074},
 acmid = {1866074},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {multitouch, tactile feedback, touch screens}
} 

@inproceedings{Khurelbaatar2016,
 author = {Khurelbaatar, Sugarragchaa and Nakai, Yuriko and Okazaki, Ryuta and Yem, Vibol and Kajimoto, Hiroyuki},
 title = {{Tactile Presentation to the Back of a Smartphone with Simultaneous Screen Operation}},
 booktitle = {Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '16},
 year = {2016},
 isbn = {978-1-4503-3362-7},
 location = {Santa Clara, California, USA},
 pages = {3717--3721},
 numpages = {5},
 url = {http://doi.acm.org/10.1145/2858036.2858099},
 doi = {10.1145/2858036.2858099},
 acmid = {2858099},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {electro-tactile display, smartphone, tactile feedback}
} 

@inproceedings{Liao2016,
 author = {Liao, Yi-Chi and Chen, Yi-Ling and Lo, Jo-Yu and Liang, Rong-Hao and Chan, Liwei and Chen, Bing-Yu},
 title = {{EdgeVib: Effective Alphanumeric Character Output Using a Wrist-Worn Tactile Display}},
 booktitle = {Proceedings of the 29th Annual Symposium on User Interface Software and Technology},
 series = {UIST '16},
 year = {2016},
 isbn = {978-1-4503-4189-9},
 location = {Tokyo, Japan},
 pages = {595--601},
 numpages = {7},
 url = {http://doi.acm.org/10.1145/2984511.2984522},
 doi = {10.1145/2984511.2984522},
 acmid = {2984522},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {alphanumerical character output, spatiotemporal vibrotactile pattern, wrist-worn tactile display}
} 

@article{Levesque2005,
 author = {L{\'e}vesque, Vincent and Pasquero, J{\'e}r\^{o}me and Hayward, Vincent and Legault, Maryse},
 title = {{Display of Virtual Braille Dots by Lateral Skin Deformation: Feasibility Study}},
 journal = {ACM Trans. Appl. Percept.},
 issue_date = {April 2005},
 volume = {2},
 number = {2},
 month = apr,
 year = {2005},
 issn = {1544-3558},
 pages = {132--149},
 numpages = {18},
 url = {http://doi.acm.org/10.1145/1060581.1060587},
 doi = {10.1145/1060581.1060587},
 acmid = {1060587},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Braille display, lateral skin deformation, tactile perception}
} 

@misc{Tretiakoff1977,
  title={{Electromechanical Transducer for Relief Display Panel}},
  author={Tretiakoff, O. and Tretiakoff, A.},
  url={http://www.google.ch/patents/US4044350},
  month=aug,
  note={US Patent 4,044,350}
}

@inproceedings{Karuei2011,
 author = {Karuei, Idin and MacLean, Karon E. and Foley-Fisher, Zoltan and MacKenzie, Russell and Koch, Sebastian and El-Zohairy, Mohamed},
 title = {{Detecting Vibrations Across the Body in Mobile Contexts}},
 booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
 series = {CHI '11},
 year = {2011},
 isbn = {978-1-4503-0228-9},
 location = {Vancouver, BC, Canada},
 pages = {3267--3276},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1978942.1979426},
 doi = {10.1145/1978942.1979426},
 acmid = {1979426},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {mobile applications, vibrotactile display, wearable haptics}
} 


@article{Wang2010,
author = { Qi Wang and Vincent Hayward},
title = {{Biomechanically Optimized Distributed Tactile Transducer Based on Lateral Skin Deformation}},
journal = {The International Journal of Robotics Research},
volume = {29},
number = {4},
pages = {323-335},
year = {2010},
doi = {10.1177/0278364909345289},
URL = {http://dx.doi.org/10.1177/0278364909345289}
}

@INPROCEEDINGS{Benali2004,
author = {Mohamed Benali-khoudja and Moustapha Hafez and Jean-marc Alex and Abderrahmane Kheddar},
title = {{Tactile Interfaces: a State-of-the-Art Survey}},
booktitle = {Int. Symposium on Robotics},
year = {2004},
pages = {721--726}
}

@inproceedings{Prescher2010,
 author = {Prescher, Denise and Weber, Gerhard and Spindler, Martin},
 title = {{A Tactile Windowing System for Blind Users}},
 booktitle = {Proceedings of the 12th International ACM SIGACCESS Conference on Computers and Accessibility},
 series = {ASSETS '10},
 year = {2010},
 isbn = {978-1-60558-881-0},
 location = {Orlando, Florida, USA},
 pages = {91--98},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/1878803.1878821},
 doi = {10.1145/1878803.1878821},
 acmid = {1878821},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {blind user, braille, gesture interaction, planar tactile display, screen reader, tactile graphics}
} 

@inproceedings{Pasquero2011,
 author = {Pasquero, Jerome and Stobbe, Scott J. and Stonehouse, Noel},
 title = {{A Haptic Wristwatch for Eyes-free Interactions}},
 booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
 series = {CHI '11},
 year = {2011},
 isbn = {978-1-4503-0228-9},
 location = {Vancouver, BC, Canada},
 pages = {3257--3266},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1978942.1979425},
 doi = {10.1145/1978942.1979425},
 acmid = {1979425},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {eyes-free interaction, haptic interface, non-visual gestures, wearable computing}
} 

@article{Benali-Khoudja2007,
author    = {Mohamed Benali{-}Khoudja and
               Moustapha Hafez and
               Abderrahmane Kheddar},
title     = {{VITAL: An electromagnetic integrated tactile display}},
journal   = {Displays},
volume    = {28},
number    = {3},
pages     = {133--144},
year      = {2007},
url       = {http://dx.doi.org/10.1016/j.displa.2007.04.013},
doi       = {10.1016/j.displa.2007.04.013},
biburl    = {http://dblp.uni-trier.de/rec/bib/journals/displays/Benali-KhoudjaH07}
}

@article{Gallo2015,
title = {{A Flexible Multimodal Tactile Display for Delivering Shape and Material Information}},
journal = "Sensors and Actuators A: Physical ",
volume = "236",
number = "",
pages = "180 - 189",
year = "2015",
note = "",
issn = "0924-4247",
doi = "http://dx.doi.org/10.1016/j.sna.2015.10.048",
url = "http://www.sciencedirect.com/science/article/pii/S0924424715302090",
author = {Simon Gallo and Choonghyun Son and Hyunjoo Jenny Lee and Hannes Bleuler and Il-Joo Cho}
}

@article{Koo2008,
 author = {Koo, Ig Mo and Jung, Kwangmok and Koo, Ja Choon and Nam, Jae-Do and Lee, Young Kwan and Choi, Hyouk Ryeol},
 title = {{Development of Soft-Actuator-Based Wearable Tactile Display}},
 journal = {Trans. Rob.},
 issue_date = {June 2008},
 volume = {24},
 number = {3},
 month = jun,
 year = {2008},
 issn = {1552-3098},
 pages = {549--558},
 numpages = {10},
 url = {http://dx.doi.org/10.1109/TRO.2008.921561},
 doi = {10.1109/TRO.2008.921561},
 acmid = {2212147},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
 keywords = {Electroactive polymer (EAP), tactile display, wearable}
} 

@inproceedings{Cauchard2016,
 author = {Cauchard, Jessica R. and Cheng, Janette L. and Pietrzak, Thomas and Landay, James A.},
 title = {{ActiVibe: Design and Evaluation of Vibrations for Progress Monitoring}},
 booktitle = {Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '16},
 year = {2016},
 isbn = {978-1-4503-3362-7},
 location = {Santa Clara, California, USA},
 pages = {3261--3271},
 numpages = {11},
 url = {http://doi.acm.org/10.1145/2858036.2858046},
 doi = {10.1145/2858036.2858046},
 acmid = {2858046},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {tactile display, tactons, vibrotactile icons},
} 

@inproceedings{Zarate2017,
	author = {Zarate, Juan Jose and Gudozhnik, Olexandr and Ruch, Anthony S{\'e}bastien and Shea, Herbert},
	title = {{Keep in Touch: Portable Haptic Display with 192 High Speed Taxels}},
	booktitle = {Proceedings of the 2017 CHI Conference Extended Abstracts on Human Factors in Computing Systems},
	series = {CHI EA '17},
	year = {2017},
	isbn = {978-1-4503-4656-6},
	location = {Denver, Colorado, USA},
	pages = {349--352},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/3027063.3052957},
	doi = {10.1145/3027063.3052957},
	acmid = {3052957},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {electromagnetic actuators, haptic display, serious gaming, taxel array}
}

@article{Zarate2016, 
author={Juan Jos\'e Z\'arate and  Herbert Shea}, 
journal={IEEE Transactions on Haptics}, 
title={{Using Pot-Magnets to Enable Stable and Scalable Electromagnetic Tactile Displays}}, 
year={2017}, 
volume={10}, 
number={1}, 
pages={106-112}, 
keywords={Actuators;Coils;Force;Magnetic flux;Magnetic noise;Magnetic shielding;Manganese;Electromagnetic forces;haptic interfaces;magnetic actuator array;magnetic shielding;planar coils array;pot-magnets}, 
doi={10.1109/TOH.2016.2591951}, 
ISSN={1939-1412}, 
month={Jan}
}

@article{Zarate2015,
title = {{Optimization of the Force and Power Consumption of a Microfabricated Magnetic Actuator}},
journal = "Sensors and Actuators A: Physical ",
volume = "234",
number = "",
pages = "57 - 64",
year = "2015",
note = "",
issn = "0924-4247",
doi = "http://dx.doi.org/10.1016/j.sna.2015.08.007",
url = "http://www.sciencedirect.com/science/article/pii/S0924424715300996",
author = {Juan Jos\'e Z\'arate and Giordano Tosolini and Simona Petroni and Massimo De Vittorio and Herbert Shea}
}


@inproceedings{Brewster2004,
 author = {Brewster, Stephen and Brown, Lorna M.},
 title = {{Tactons: Structured Tactile Messages for Non-visual Information Display}},
 booktitle = {Proceedings of the Fifth Conference on Australasian User Interface - Volume 28},
 series = {AUIC '04},
 year = {2004},
 location = {Dunedin, New Zealand},
 pages = {15--23},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=976310.976313},
 acmid = {976313},
 publisher = {Australian Computer Society, Inc.},
 address = {Darlinghurst, Australia, Australia},
 keywords = {Tactons, multimodal interaction, non-visual cues, tactile displays}
} 

@inproceedings{Luk2006,
 author = {Luk, Joseph and Pasquero, Jerome and Little, Shannon and MacLean, Karon and Levesque, Vincent and Hayward, Vincent},
 title = {{A Role for Haptics in Mobile Interaction: Initial Design Using a Handheld Tactile Display Prototype}},
 booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
 series = {CHI '06},
 year = {2006},
 isbn = {1-59593-372-7},
 location = {Montr\&\#233;al, Qu\&\#233;bec, Canada},
 pages = {171--180},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1124772.1124800},
 doi = {10.1145/1124772.1124800},
 acmid = {1124800},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {design process, display, handheld interaction, haptic, lateral skin stretch, mobile, multimodal, tactile}
} 

@INPROCEEDINGS{Morrow2016, 
author={K. Morrow and D. Wilbern and R. Taghavi and M. Ziat}, 
booktitle={2016 IEEE Haptics Symposium (HAPTICS)}, 
title={{The Effects of Duration and Frequency on the Perception of Vibrotactile Stimulation on the Neck}}, 
year={2016}, 
pages={41-46}, 
keywords={biomedical equipment;touch (physiological);visual perception;duration effects;frequency effects;impact performance;perception;tactile directional information;vestibular loss;viable location;vibrotactile neck device;vibrotactile stimulation;Legged locomotion;Muscles;Neck;Shape;Training;Vibrations;Visualization}, 
doi={10.1109/HAPTICS.2016.7463153}, 
month={April}
}

@inproceedings{Lindsay2013,
 author = {Lindsay, Jack I.C. and Jiang, Iris and Larson, Eric and Adams, Richard and Patel, Shwetak N. and Hannaford, Blake},
 title = {{Good Vibrations: An Evaluation of Vibrotactile Impedance Matching for Low Power Wearable Applications}},
 booktitle = {Proceedings of the 26th Annual ACM Symposium on User Interface Software and Technology},
 series = {UIST '13},
 year = {2013},
 isbn = {978-1-4503-2268-3},
 location = {St. Andrews, Scotland, United Kingdom},
 pages = {515--520},
 numpages = {6},
 url = {http://doi.acm.org/10.1145/2501988.2502051},
 doi = {10.1145/2501988.2502051},
 acmid = {2502051},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {haptics, vibration motors, vibrotactile}
} 

@article{Weinstein1968,
author={Weinstein, S},
title={{Intensive and Extensive Aspects of Tactile Sensitivity as a Function of Body Part, Sex and Laterality}},
journal={{Kenshalo. The Skin Senses}},
ISSN={},
publisher={Charles C. Thomas},
year={1968},
month={},
volume={},
number={},
pages={195--222},
DOI={}
}

@article{Penfield1950,
title= {{The Cerebral Cortex of Man: a Clinical Study of Localization of Function}} ,
author={Penfield, Wilder and Rasmussen, author = {Penfield, Wilder and Rasmussen, Theodore},
},
journal = {Journal of the American Medical Association},
volume = {144},
number = {16},
pages = {1412},
year = {1950},
doi = {10.1001/jama.1950.02920160086033}
}

@inproceedings{Poupyrev2016,
 author = {Poupyrev, Ivan and Gong, Nan-Wei and Fukuhara, Shiho and Karagozler, Mustafa Emre and Schwesig, Carsten and Robinson, Karen E.},
 title = {{Project Jacquard: Interactive Digital Textiles at Scale}},
 booktitle = {Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '16},
 year = {2016},
 isbn = {978-1-4503-3362-7},
 location = {Santa Clara, California, USA},
 pages = {4216--4227},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2858036.2858176},
 doi = {10.1145/2858036.2858176},
 acmid = {2858176},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {information interfaces and presentation}
}

@inproceedings{Saket2013,
 author = {Saket, Bahador and Prasojo, Chrisnawan and Huang, Yongfeng and Zhao, Shengdong},
 title = {{Designing an Effective Vibration-based Notification Interface for Mobile Phones}},
 booktitle = {Proceedings of the 2013 Conference on Computer Supported Cooperative Work},
 series = {CSCW '13},
 year = {2013},
 isbn = {978-1-4503-1331-5},
 location = {San Antonio, Texas, USA},
 pages = {149--1504},
 numpages = {1356},
 url = {http://doi.acm.org/10.1145/2441776.2441946},
 doi = {10.1145/2441776.2441946},
 acmid = {2441946},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {alerts, mobile phone, notifications, perceived urgency, vibration patterns}
} 

@inproceedings{Alvina2015,
 author = {Alvina, Jessalyn and Zhao, Shengdong and Perrault, Simon T. and Azh, Maryam and Roumen, Thijs and Fjeld, Morten},
 title = {{OmniVibe: Towards Cross-body Spatiotemporal Vibrotactile Notifications for Mobile Phones}},
 booktitle = {Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
 series = {CHI '15},
 year = {2015},
 isbn = {978-1-4503-3145-6},
 location = {Seoul, Republic of Korea},
 pages = {2487--2496},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/2702123.2702341},
 doi = {10.1145/2702123.2702341},
 acmid = {2702341},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {arm, mobile device, notification, palm, spatiotemporal vibrotactile pattern, tactile feedback, thigh, waist},
} 

@inproceedings{King2010,
 author = {King, H Hawkeye and Donlin, Regina and Hannaford, Blake},
 title = {{Perceptual Thresholds for Single vs. Multi-Finger Haptic Interaction}},
 booktitle = {Proceedings of the 2010 IEEE Haptics Symposium},
 series = {HAPTIC '10},
 year = {2010},
 isbn = {978-1-4244-6821-8},
 pages = {95--99},
 numpages = {5},
 url = {http://dx.doi.org/10.1109/HAPTIC.2010.5444670},
 doi = {10.1109/HAPTIC.2010.5444670},
 acmid = {2192763},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
 keywords = {single finger devices, perceptual thresholds, single finger haptic interaction, multifinger haptic interaction, psychophysical thresholds, multifinger single point interaction, haptic effects, UW multifinger haptic display, haptic icons, virtual environment, forced-choice adaptive thresholding method, detectable force magnitude, force detection threshold, analysis of variance, t-tests, Bonferroni correction, multifinger device parameters}
} 

@article{Dosher2005,
 author = {Dosher, Jesse and Hannaford, Blake},
 title = {{Human Interaction with Small Haptic Effects}},
 journal = {Presence: Teleoper. Virtual Environ.},
 issue_date = {June 2005},
 volume = {14},
 number = {3},
 month = jun,
 year = {2005},
 issn = {1054-7460},
 pages = {329--344},
 numpages = {16},
 url = {http://dx.doi.org/10.1162/105474605323384672},
 doi = {10.1162/105474605323384672},
 acmid = {1149682},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA}
} 

@Article{Louw2002,
author={Louw, S. and Kappers, A. M. L. and Koenderink, J. J.},
title={{Active Haptic Detection and Discrimination of Shape}},
journal="Perception {\&} Psychophysics",
year="2002",
volume="64",
number="7",
pages="1108--1119",
abstract="In previous research, we have shown that detection thresholds for Gaussian shapes increase with a power of 1.3 of spatial width. In the present three experiments, we generalized this finding to more complex shapes and to discrimination tasks. In Experiment 1, we found that the slope of the psychometric function for detection (i.e., distinguishing curved from flat surfaces) was independent of surface shape. In Experiment 3, we found the same result for discrimination of two different curved shapes. In Experiment 2, we found that detection and discrimination functions had the same dependence on spatial width, except that discrimination thresholds were two to four times larger. Possible neural mechanisms underlying these results are discussed.",
issn="1532-5962",
doi="10.3758/BF03194760",
url="http://dx.doi.org/10.3758/BF03194760"
}

@article{Hirsh1961,
  author = {Hirsh, I. J. and Jr, C. E. Sherrick},
  biburl = {https://www.bibsonomy.org/bibtex/218c380a994bd270f34ce11b6deedf073/sourcefilter},
  journal = {Journal of Experimental Psychology},
  keywords = {imported},
  pages = {423--432},
  timestamp = {2009-04-01T22:43:24.000+0200},
  title = {{Perceived order in different sense modalities}},
  volume = {62},
  year = {1961}
}

@article{Chancey2014,
author = {Eric T. Chancey and J. Christopher Brill and Adam Sitz and Ulrike Schmuntzsch and James P. Bliss},
title = {{Vibrotactile Stimuli Parameters on Detection Reaction Times}},
journal = {Proceedings of the Human Factors and Ergonomics Society Annual Meeting},
volume = {58},
number = {1},
pages = {1701-1705},
year = {2014},
doi = {10.1177/1541931214581355},
URL = {http://dx.doi.org/10.1177/1541931214581355},
eprint = {http://dx.doi.org/10.1177/1541931214581355}
}

@inproceedings{Brown2006,
 author = {Brown, Lorna M. and Brewster, Stephen A. and Purchase, Helen C.},
 title = {{Multidimensional Tactons for Non-visual Information Presentation in Mobile Devices}},
 booktitle = {Proceedings of the 8th Conference on Human-computer Interaction with Mobile Devices and Services},
 series = {MobileHCI '06},
 year = {2006},
 isbn = {1-59593-390-5},
 location = {Helsinki, Finland},
 pages = {231--238},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/1152215.1152265},
 doi = {10.1145/1152215.1152265},
 acmid = {1152265},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {non-visual interaction, tactile displays, tactile icons, tactons},
} 

@inproceedings{Schneider2016,
 author = {Schneider, Oliver S. and Seifi, Hasti and Kashani, Salma and Chun, Matthew and MacLean, Karon E.},
 title = {{HapTurk: Crowdsourcing Affective Ratings of Vibrotactile Icons}},
 booktitle = {Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '16},
 year = {2016},
 isbn = {978-1-4503-3362-7},
 location = {Santa Clara, California, USA},
 pages = {3248--3260},
 numpages = {13},
 url = {http://doi.acm.org/10.1145/2858036.2858279},
 doi = {10.1145/2858036.2858279},
 acmid = {2858279},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {crowdsource, design, haptic, mechanical turk, multimodal, user study, vibrotactile, visualization}
} 

@inproceedings{Dobbelstein2016,
 author = {Dobbelstein, David and Henzler, Philipp and Rukzio, Enrico},
 title = {{Unconstrained Pedestrian Navigation Based on Vibro-tactile Feedback Around the Wristband of a Smartwatch}},
 booktitle = {Proceedings of the 2016 CHI Conference Extended Abstracts on Human Factors in Computing Systems},
 series = {CHI EA '16},
 year = {2016},
 isbn = {978-1-4503-4082-3},
 location = {Santa Clara, California, USA},
 pages = {2439--2445},
 numpages = {7},
 url = {http://doi.acm.org/10.1145/2851581.2892292},
 doi = {10.1145/2851581.2892292},
 acmid = {2892292},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {pedestrian navigation, vibro-tactile, watch, wrist}
} 

@inproceedings{Tsukada2004,
author= {Tsukada, Koji and Yasumura, Michiaki},
editor= {Davies, Nigel and Mynatt, Elizabeth D. and Siio, Itiro},
title= {{ActiveBelt: Belt-Type Wearable Tactile Display for Directional Navigation}},
bookTitle= { Proceedings of UbiComp 2004: Ubiquitous Computing: 6th International Conference},
year= {2004},
location = {Nottingham, UK},
publisher= {Springer Berlin Heidelberg},
address= {Berlin, Heidelberg},
pages= {384--399},
numpages = {15},
isbn= {978-3-540-30119-6},
doi= {10.1007/978-3-540-30119-6_23}
}

==> chapters/04_joint_interfaces/content/conclusion.tex <==
\chapter{Summary \& Insights}
\label{ch:shared:conclusion}

\paragraph{Summary}
We introduced two novel electromagnetic platforms designed to actuate a permanent magnet in the surrounding space. The first project, "\omniHapTitle" (\chapref{ch:shared:contact}), focused on designing and fabricating a spherical electromagnet capable of generating adjustable radial and tangential forces using three orthogonal electromagnetic coils integrated into a single sphere. This system targets a handheld tool, such as a stylus, and allows users to feel relatively large forces despite the tool being untethered. A user experiment with six participants characterized the force delivery and perceived precision, revealing a resolution of at least 25 discernible locations for repelling forces distributed across the hemisphere. However, \omniHap required external tracking of the tool, which was cumbersome and expensive.

In "\omniUISTTitle" (\chapref{ch:shared:volumetric}), we addressed the tracking limitation of \omniHap by integrating 3D magnetic sensing using Hall sensors with magnetic actuation through an improved spherical electromagnet. This integration allows spatial interaction systems to incorporate 3D tracking and actuation of untethered tools by embedding a small permanent magnet. The core contribution of \omniUIST is resolving the interference caused by simultaneous magnetic tracking and actuation using a novel gradient-based optimization method. This method provides 3D tracking capabilities with a mean error of 6.9 mm during actuation forces of up to 2N. We demonstrated several example applications showcasing \omniUIST's capabilities.

\paragraph{Implications}
In our context, both the user and the system interact with a shared variable, such as car acceleration or a graphical menu. Kinesthetic haptic feedback is a special case where this variable (e.g., joystick position) is both acted upon and perceived through the same modality, like the user's hands. Previous research on kinesthetic haptic feedback generally focuses on complex mechanical devices (e.g., \cite{Massie94, Stamper1997, VanDerLinde2002, Araujo2016, zoller2019assessment, Sinclair2019Capstan}). Extensions of these systems include exoskeletons~\cite{Gu2016, Choi2016}, gloves~\cite{Cybergrasp, hinchet2018dextres}, and tilt-platforms~\cite{Prattichizzo2013, Kim2016}. However, these often necessitate user instrumentation and introduce system friction that users can always feel, even when the system is off, thereby limiting full user control.

In contrast, our work provides grounded yet untethered forces onto a tool, thereby overcoming the limitations of not covering the full spectrum from user agency to system automation. Our work lays the foundation for investigating haptic devices from a new perspective, that of shared variable interfaces. We have taken the first step towards understanding these interfaces, demonstrating that haptic shared variable interfaces open up novel applications in gaming, object exploration, and design. By eliciting forces on the tool manipulated by the user, we enable haptic feedback in the same modality as the user's exertion, resulting in natural interactions. This integration of sensing and actuating the tool through electromagnetism is both cost-effective and efficient.

\paragraph{Limitations}
Both \omniHap and \omniUIST have limitations within the context of interfaces with shared variables.

First, while our work suggests that interacting with a shared variable haptic interface is natural for users, it remains uncertain to what extent our findings generalize to other interface types, such as graphical interfaces. Further investigation is needed to understand the interaction implications beyond the haptic paradigm.

Second, we have not compared our results to haptic feedback without a shared variable, such as vibrotactile feedback. Comparing against a broader range of haptic devices would allow us to draw more comprehensive conclusions regarding usability improvements.

Finally, we have not explored an optimal control strategy for haptic feedback. Haptic feedback involves not only the device itself but also how the device is controlled. Currently, we provide haptic feedback based on heuristics and the current tool position. An adaptive strategy incorporating a predictive user model might be more effective. Such a control method could balance autonomy and automation, and account for user intent, making the device more dynamic.

==> chapters/04_joint_interfaces/content/introduction.tex <==
\chapter{Introduction}
\label{ch:shared:introduction}
% Shared Variable
Contextual intelligent systems often work with and alongside humans. Their contextual nature allows them to make decisions based on more variables than just explicit user input (i.e., context). This loop of observing the world, decision-making, and acting in the world is similar to human actions. Since both humans (natural agents) and intelligent systems (artificial agents) can operate in the real world simultaneously, this world becomes a shared medium of communication between both agents (see Fig. \ref{fig:enter-label}). The user can change something that impacts the perception and decision-making of the artificial agent, and vice versa. However, not all contextual variables in the world are shared between both agents, due to differences in perceptual capabilities, tasks, or interests. Hence, a subset of all contextual variables is a shared variable, meaning a variable that both agents can perceive and that influences the decision-making process.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{example-image-a}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

% --> Haptics
A specific instance of a shared variable interface is a subset of haptic interfaces. Haptic interfaces are particularly interesting because they operate in the physical world, where the challenge of variable ownership is much more impactful. Additionally, two agents exerting force on a single object is an intuitive way to consider shared variable interfaces. For a haptic device to have a shared variable, it generally needs to fulfill two prerequisites. First, as the term interface indicates, the haptic device must function as both an input and output device. While many haptic devices function primarily as output devices (such as Dextres \cite{hinchet2018dextres}), some can also serve as input devices. Second, the haptic feedback it provides should be kinesthetic rather than (vibro-)tactile. Haptic interfaces that fulfill both criteria are characterized by their ability to affect a shared variable through interaction, either by restricting hand movement or by actively moving a tool. For physically based interactions, as in haptics, this means delivering a force.

% Content
%% 1
We investigate a haptic shared variable interface through a use case, presented in two chapters. In the first chapter (\ref{}), we discuss the design and fabrication of a contact-free volumetric haptic feedback device. Our device is a novel spherical electromagnetic system that delivers grounded, yet untethered, forces on a tool. The device consists of a single 60 mm diameter spherical electromagnet and can render attractive and repulsive forces onto permanent magnets embedded in pointing tools such as a stylus or magnets directly worn on the user’s fingertip. Leveraging a dipole-dipole approximation of the electromagnet-magnet interaction, our system is capable of calculating and controlling the forces exerted on the permanent magnet in real-time while dynamically adjusting the force perceived by the user. The system can deliver perceptible forces up to 1N in a thin volume above the surface. Furthermore, we demonstrate that users can distinguish at least 25 different set-points separated by $18^\circ$ on the surface of the sphere. Our device builds on three key components that represent our contributions in this work: i) A computational model based on magnetic dipole-dipole interaction to produce force maps that allow for designing and generating location-dependent feedback, ii) the design and implementation of a 3 degree-of-freedom (DoF) spherical electromagnet prototype, and iii) a control strategy that translates desired high-level forces into low-level input signals (currents/voltages) for the coils, fast enough for interactive use.

%% 2
In the second chapter (\ref{}), we present Omni, a self-contained 3D haptic feedback system capable of sensing and actuating an untethered, passive tool containing only a small embedded permanent magnet. The electromagnetic actuation and sensing interfere since two physical phenomena (e.g., tool motion and electromagnet control) create a single, superimposed magnetic field. To decompose the resulting superposition of magnetic fields, we introduce a novel 3D positioning algorithm. Our formulation reconstructs the magnet’s 3D position by minimizing the residual between the predicted magnetic field strength at a given location and the actual measurement picked up by the Hall sensors. The formulation is amenable to gradient-based optimization, and we show that the problem can be solved via a quasi-Newton solver in real-time. We make the following contributions in this project: i) a fully self-contained system, combining actuation and tracking components, ii) a novel algorithm for the reconstruction of the 3D tool position under electromagnetic actuation, iii) a thorough technical evaluation of the algorithm, yielding an accuracy of 5 mm without actuation and 7 mm with the electromagnet on, iv) assessment of the force generation capabilities, showing up to 2 N of haptic force in any direction, and v) an exploration of use cases afforded by Omni.

% Implications
The implications of our investigation into haptic shared variable interfaces are two-fold. First, we show that shared variable interfaces open up novel applications in areas such as gaming, object exploration, and design. Second, we show that manipulating the same device is natural for the user. Sensing and actuating the same device is necessary for this. Doing this via the same modality, electromagnetism in this case, is a cost-effective and efficient solution.

% Summary
In summary, we introduce two novel electromagnetic platforms that actuate a permanent magnet in the space around it. In the first project, we focus on the design and fabrication of a spherical electromagnet. We used this to inform the second project, Omni. Omni integrates 3D magnetic sensing using Hall sensors and magnetic actuation through radial and tangential forces produced by three orthogonal electromagnetic coils integrated into a single sphere. Omni’s capabilities allow spatial interaction systems to integrate 3D tracking and actuation of untethered, free-ranging tools, simply by embedding a small permanent magnet. We can use our findings as a starting point for investigating shared variable interfaces. 

==> chapters/04_joint_interfaces/sensing/sections/00_abstract.tex <==
\begin{abstract}
% JZ:
% - method for tracking magnets in the 3D space
% - 
% 
% In this paper we propose a gradient-based method to track a permanent magnet in 3D space, while simultaneously exerting electromagnetic forces onto the permanent magnet. Being able to track the magnet, embedded in a tool, enables more compact, accessible haptic feedback devices that are self-contained. As a proof of concept a circular array of hall sensors and a spherical electromagnet are combined to create a novel haptic feedback device. This device is thoroughly technically evaluated from both an actuating as well as sensing perspective. We find that we actuate with a force of at least ..N on ... different points in a shell above the electromagnet. In the same shell, we can track the pen with an accuracy of ...mm, this equates in ... number of zones in which we can disinguish the pen position. Finally, we show the merit of our method by showcasing a variety of applications, including exploring the viscosity of liquids, designing 3d shapes and playing games.  



% In this paper, we proposed a self-contained haptic feedback system that is capable of sensing, and actuating on, a permanent magnet.  
% Being able to track a permanent magnet in 3D space, while simultaneously exerting an electromagnetic force, has been a long-standing problem. We propose a gradient-based tracking method, in combination with eight affordable off-the-shelf hall sensors, to sense the position of a permanent magnet embedded in 3D printed tool. The hall sensors are located in a circular array around a spherical electromagnet. The electromagnet is capable of exerting significant forces with a large accuracy in a volumetric space around the system. Since the system is self-contained, and therefore not reliant on external systems,  it is easy and affordable to fabricate, making it accessible to a large audience. While providing haptic feedback, the tracking is accurate enough for most use-cases. Next to a thorough technical evaluation, we demonstrate a large variety of applications.

% #######################
% ABSTRACT OTMAR & CHRISTIAN, MERGED BY DL
% ####################### 



% We present Omni, a self-contained 3D haptic feedback system that is capable of \emph{sensing} and \emph{actuating} an untethered, passive tool containing only a small embedded permanent magnet.
% %
% Omni enriches VR, AR and desktop applications by providing an active haptic experience using a simple apparatus centered around an electromagnetic base. 
% %
% The spatial haptic capabilities of Omni are enabled by a novel gradient-based method to estimate the 3D position of the permanent in midair through eight small off-the-shelf hall sensors that are integrated into the base.
% %
% Omni's 3 DoF spherical electromagnet \textit{simultaneously} exerts dynamic and precise radial and tangential forces in a volumetric space around the device. 
% %
% %%%Notably, the amount of exerted force depends solely on the volume of the magnet inserted in the tool, and not its distance to the base of the device. 
% %
% Since our system is fully integrated and requires no external tracking, it is easy and affordable to fabricate, and because it contains no moving parts it can be very robust.
% %
% We describe Omni's implementation, its software control, and evaluate its tracking and actuation quality, as well as a series of use-cases and applications demonstrating its capabilities.
%
% #######################
% ABSTRACT OTMAR
% ####################### 

% In this paper, we propose a self-contained haptic feedback system that is capable of \emph{sensing} and \emph{actuating} an untethered, passive  tool containing only a permanent magnet, without requiring any external tracking equipment and thus admitting for a compact form-factor.  
% %
% The system can sense rich interaction and provide haptic feedback in the context of VR, AR or desktop applications in order to increase immersion.
% %
% To locate the handheld tool, the measurements of eight off-the-shelf hall sensors are integrated in a gradient-based optimization scheme to accurately track the position of a permanent magnet that moves in the midair.
% %
% In turn, a 3 DoF spherical electromagnet provides precise and dynamic force feedback in a volumetric space around the device. 
% The amount of exerted force depends on the volume of the magnet inserted in the tool, for which we provide thorough analysis and design guidelines.
% %
% Since the system is self-contained, and therefore not reliant on external systems, it is easy and affordable to fabricate, making it accessible to a broad audience. 
% %
% While providing haptic feedback, the tracking is fast and accurate enough for most use-cases. Next to a thorough technical evaluation, we demonstrate a large variety of applications.



% #######################
% ABSTRACT CHRISTIAN
% #######################

% We present NAME, a self-contained haptic feedback system that can track and actuate freely movable tools around it in 3D aided by a small embedded permamagnet.
% NAME complements VR, AR and desktop applications with convincing haptic experiences using a simple apparatus centered around an electromagnet base.
% What enables NAME's spatial haptic capabilities is our novel gradient-based method to estimate the 3D position of the permanent in midair through eight small hall sensors.
% % CH: is it really force feedback or actually an actuation? E.g., is it in response to an input force? I think it's even more general than just 'pushing back'
% Through the same modality, NAME's 3 DoF spherical electromagnet exerts dynamic and precise radial and tangential forces that, notably, are independent of the permamagnet's distance up to a certain boundary. 
% Our system is fully integrated and requires no external tracking, which makes fabrication quick and affordable and will allow NAME to be an accessible haptic feedback apparatus for a broad audience.

% We describe NAME's implementation, its software control, and evaluate the tracking and actuation qualitney depending on used magnet volumes.
% For example, NAME can track a (4\,mm)$^3$ permamagnet accurately within $\pm$ X\,mm accuracy at X\,fps. 
% We demonstrate a series of use-cases of our system and conclude with design guidelines for future applications.

\end{abstract}

==> chapters/04_joint_interfaces/sensing/sections/01_introduction.tex <==
\section{Introduction}
This chapter builds on \omniHapTitle (\chapref{ch:shared:contact}), by presenting \omniUIST, a self-contained 3D haptic feedback system. We enhance \omniHap in two significant ways: first, by improving the actuator to enable increased peak and continuous forces, and second, by integrating sensing to overcome the limitations of expensive and cumbersome external tracking.

One of the core challenges in enabling high-fidelity free-space haptic interactions is to reliably track the input device in space while \emph{simultaneously} exerting forces. While optical tracking systems can be used for 3D localization, they require significant instrumentation of the user's environment, making them impractical for real-world deployments.

To address this challenge, we propose \omniUIST, an integrated system that can locate the tool in free space and deliver finely controllable haptic feedback via the same modality. Our system consists of an omnidirectional spherical electromagnet that delivers attractive and repulsive forces in radial and tangential directions onto a small, handheld magnet (\figref{fig:teaser_sensing}).

To track the tool's location, we leverage eight integrated Hall sensors positioned in two separate XY-planes relative to the electromagnet's coils. These sensor readings allow us to reconstruct the tool's position based on the distortion of the magnetic field caused by the tool's motion. Unlike previous approaches that rely on passive magnets \cite{ashbrook2011nenya, liang2012gausssense}, our setting is more challenging due to the use of an active electromagnet. The electromagnetic actuation and sensing interfere, creating a superimposed magnetic field.

To decompose this superposition of magnetic fields, we introduce a novel 3D positioning algorithm. Our formulation reconstructs the magnet's 3D position by minimizing the residual between the predicted magnetic field strength at a given location and the actual measurements from the Hall sensors. This approach is amenable to gradient-based optimization, and we demonstrate that the problem can be solved in real-time using a quasi-Newton solver, achieving an accuracy of 6.9mm after a one-shot calibration procedure.

We demonstrate the capabilities of our approach through a series of interactive use cases, some shown in \figref{fig:usecases}, leveraging the ability to track the handheld tool in 3D while simultaneously delivering dynamically adjustable haptic feedback. The magnet fits inside passive tools, such as a 3D-printed stylus, supporting fine-grained interaction tasks and alternative uses as a joystick. We showcase applications in gaming, accessibility, mixed reality, and 3D CAD design that utilize \omniUIST's 3D tracking and actuation.

We detail our software and hardware implementation and thoroughly assess \omniUIST's sensing and actuation capabilities. Our findings indicate that \omniUIST can continuously deliver up to 0.6N in any direction near the sphere, with the electromagnetic coils heating up to a sustainable 47°C. The system's peak force reaches 1.8N for repelling and -3.1N for attractive forces to the sphere, and ±2N in the tangential plane. \omniUIST can actuate the magnet at 100Hz and sense and estimate its 3D position at 40Hz.

In summary, this chapter makes the following contributions:
\begin{itemize}
\item A fully self-contained system combining actuation and tracking components,
\item A novel algorithm for the reconstruction of the 3D tool position under electromagnetic actuation,
\item A thorough technical evaluation of the algorithm, achieving an accuracy of 5mm without actuation and 7mm with the electromagnet on,
\item An assessment of the force generation capabilities, demonstrating up to 2N of haptic force in any direction,
\item An exploration of use cases enabled by \omniUIST.
\end{itemize}
Our method can be extended to any apparatus involving a permanent magnet, integrating spatial position reconstruction and spatial actuation into a single device.

==> chapters/04_joint_interfaces/sensing/sections/02_related_work.tex <==




==> chapters/04_joint_interfaces/sensing/sections/03_method_old.tex <==
\section{Method}
\subsection{Hardware}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/hardware_try.png}
    \caption{Hardware Overview}
    \label{fig:hardware}
\end{figure}
electronics, size, FEM, informed design, 


\begin{figure*}[!h]
    \centering
    \includegraphics[width=\textwidth]{figures/hardware2.pdf}
    \caption{Hardware Overview}
    \label{fig:hardware}
\end{figure*}

\subsection{Input Sensing}
\begin{figure}
    \centering
    \includegraphics{sections/coordinates.pdf}
    \caption{Coordinate System Used}
    \label{fig:coordinates}
\end{figure}

In general, it is straight-forward to compute the magnetic field at an arbitrary position $\mathbf{B}(\mathbf{r})$:
\begin{equation}
    \mathbf {B} (\mathbf {r} )={\frac {\mu _{0}}{4\pi }}{\frac {3\mathbf {\hat {r}} (\mathbf {\hat {r}} \cdot \mathbf {m} )-\mathbf {m} }{|\mathbf {r} |^{3}}}.
    \label{eq:basic_B}
\end{equation}
given that $r$ is the vector from the center of the magnet to the arbitrary location, $\mu_0$ is the relative permeability of a vacuum and $m$ is the magnetic moment we can be expressed for both permanent magnets as well as electromagnets. 

However, it is impossible to inverse this function. Making a closed-form solution to find a magnet position (expressed in $r$) given $\mathbf{B}(\mathbf{r})$ and $\mathbf{m}$ intractable. However, we are interested in finding position $\mathbf{P}$ of a permanent magnet, a further complication is that the actuation of our spherical electromagnet also influences the magnetic field. 

In order to solve this problem we place 16 hall sensors around the input area and try to minimize the following cost-term:
\begin{equation}
    \arg\underset{\mathbf{P}, \mathbf{I}}{\min} \|\sum_i \mathbf{w}_{i} \left[(\mathbf{B}_{p,i}(\mathbf{P})+\mathbf{B}_{em,i}(\mathbf{I}) + \mathbf{B}_{n,i}) - \Tilde{\mathbf{B}}_i\right]^2 \|
    \label{eq:eneregy}
\end{equation}

\begin{equation}
    \mathbf{w}_{i} = (\Tilde{\mathbf{B}}_i/ \Tilde{\mathbf{B}}_{max})^2 \ \  
                \text{if}\ \ (\Tilde{\mathbf{B}}_i/ \Tilde{\mathbf{B}}_{max})^2 < 1,\ \ \text{else}\ \ 0
\end{equation}

where $\mathbf{B}_i$ is the magnetic field measurement in $x,y,z$-direction at hall sensor $i$. Specifically, $\mathbf{B}_p$ is the magnetic field caused by the permanent magnet in the pen as a function of its position $\mathbf{P}$ (defined as a 3-tuple: $(x,y,z)$), $\mathbf{B}_em$ by the electromagnet as a function of its input current $\mathbf{I}$, $\mathbf{B}_n$ is the noise in the environment. Given that magnetic fields obey the principle of super-position we can simply sum them. Then we try to minimize the difference between the hypothetical measurements and the actual measurements $\Tilde{\mathbf{B}}$ for each hall sensor. The hypothetical readings are based on Equation \ref{eq:basic_B}. 

We make several assumptions here. The first assumption is that all magnets behave as a dipole. The second assumption is that the tool, and therefore the permanent magnet, always points towards the center of the electromagnet. From the latter assumption it follows that the orientation of the permanent magnetic in spherical coordinates can be expressed as:

\begin{align}
    \theta &= \arctan \left( \frac{\sqrt{x^2+y^2}}{z}\right)\\
    \phi &= \arccos \left( \frac{x}{\sqrt{x^2+y^2}} \right)
\end{align}
from this we can define $\mathbf{m}_p$, which is the magnetic moment of the permanent magnetic:
\begin{align}
    \mathbf{m} &= m * \begin{bmatrix}\sin(\theta)*\cos(\phi)\\\sin(\theta)\sin(\phi)\\\cos(\theta)\end{bmatrix}\\
    m &= \frac{1}{\mu_0}*Br*V
\end{align}
where, $V$ is the volume of the permanent magnet and $Br$ is the magnetic flux density in Teslas. Given a 3-tuple for the location of the hall sensor $\mathbf{s} := \{s_x, s_y, s_z\}$ we can define $\mathbf{r}_p$:
\begin{equation}
    \mathbf{r}_p = \mathbf{s} - \mathbf{P}
\end{equation}

Given Equation \ref{eq:basic_B} and our definitions of $\mathbf{m}_p$ and $\mathbf{r}_p$ it is now trivial to compute $\mathbf{B}_p$ for each hall sensor:

\begin{equation}
        \mathbf {B}_p (\mathbf {r}_p )={\frac {\mu _{0}}{4\pi }}{\frac {3\mathbf {\hat {r}_p} (\mathbf {\hat {r}}_p \cdot \mathbf {m}_p )-\mathbf {m}_p }{|\mathbf {r}_p |^{3}}}.
        \label{eq:Bp}
\end{equation}

We can do a similar calculation for $\mathbf{B}_{em}$, since this is magnet is spherical the orientation does not matter, and since the magnet is centered around the origin of our global coordinate system $\mathbf{r}_em = \mathbf{s}$. Since we build the spherical electromagnet ourselves there are bound to be impurities and inconsistencies. Therefore, we refrain from using a theoretical model to calculate $\mathbf{m}_{em}$ and rely on a calibration matrix $C \in \mathbb{R}^{3\times3}$, which we assume linearly scales with the input current $\mathbf{I}$ so that:

\begin{equation}\label{eq:me_vs_I}
    \mathbf{m}_e =  \frac{2*\pi*I_t^{(s)}*\mathbf{d}^3}{\mathbf{c} *\mu_0}
\end{equation}

therefore,
\begin{equation}
        \mathbf {B}_{em} (\mathbf {r}_{em} )={\frac {\mu _{0}}{4\pi }}{\frac {3\mathbf {\hat {r}_{em}} (\mathbf {\hat {r}}_{em} \cdot \mathbf {m}_{em} )-\mathbf {m}_{em} }{|\mathbf {r}_{em} |^{3}}}.
        \label{eq:Be}
\end{equation}
Finally, $\mathbf{B}_n$ simply comes from a calibration and remains a constant throughout a session.

We minimize Equation \ref{eq:eneregy} in a gradient approach, where we update the six free variables found in the position of the permanent magnet and the current input in the electromagnet. In theory it is possible to directly use the input current and/or the measured current for the latter. However, in practice this infeasible due to latency and thermal drift (which alters the resistance of the coils and therefore the current supplied). Our optimization approach can be found in algorithm \ref{algo:postion}. We use pytorch due to its autograd and ready-implemented optimization schemes, which reduce overhead. Specifically we use Limited-memory BFGS, which is a quasi-newton method. It is an approximation of the BFGS, which works well on non-smooth optimization instances. 

\begin{algorithm}
\SetAlgoLined
\SetKwInOut{Output}{\textbf{Output}}
\SetKwInOut{Input}{\textbf{Input}}
\KwResult{$x,y,z$-position of permanent magnet, $x,y,z$-current of the electromagnet}

 $\mathbf{P} \leftarrow [0,0,h]$\tcp*{$h$ = distance from p to em}
 $\mathbf{I} \leftarrow [0,0,0]$\;
 $\mathbf{B}_n \leftarrow$ Calibration\;
 Loss() $\leftarrow \| (\mathbf{B}_{p}(\mathbf{P})+\mathbf{B}_{em}(\mathbf{I}) + \mathbf{B}_{n}) - \Tilde{\mathbf{B}}\|^2$\;
 \While{interaction session}{
  \Input{$\mathbf{I}_{\text{measured}}$}
  \Input{$\Tilde{\mathbf{B}}$}
  LBFGS.init($\mathbf{P}, \mathbf{I}_{\text{measured}}$)\;
  $\mathbf{P}, \mathbf{I} \leftarrow$ LBFGS.optim$(\Tilde{\mathbf{B}}, \mathbf{B}_n, \mathbf{B}_p(\mathbf{P}), \mathbf{B}_{em}(\mathbf{I}), Loss())$\;
 \Output{$\mathbf{P}$}
 }
 \caption{Permanent Magnet Position}
 \label{algo:postion}
\end{algorithm}

\begin{figure}
    \centering
    \def\svgwidth{\columnwidth}
    \includegraphics{figures/cost.pdf}
    \caption{Visual representation of the solver results. X,Y-axis are spherical coordinates, for representation purposes we omitted $r$. The Z-axis is the loss. This is one solver update, which is done in roughly 40ms and 20 iterations.}
    \label{fig:cost}
\end{figure}

Following the dipole-dipole assumption it is also straightforward to compute the forces exerted on the tool, in the coordinates of the tool:

\begin{eqnarray}
    \mathbf{F_{r}} &=& - \frac{3 \mu_0 \ m_{e} \ m_{p}}{2 \pi \ d^4} \cos(\alpha) \ \mathbf{e_{r}} \label{eq:Fr}\ ,\\ 
    \mathbf{F_{t}} &=& - \frac{3 \mu_0 \ m_{e} \ m_{p}}{4 \pi \ d^4} \sin(\alpha) \ \mathbf{e_{t}} \label{eq:Ft}\ ,
\end{eqnarray}
where $\me=|\meBold|$, $\mpp=|\mpBold|$. In the above expression, $\FrBold$ is the force in the radial direction $\RpenBold = d \ \er$ from the center of the device to the tool. Likewise, $\FtBold$ is the force in the tangential direction $\et$ that tends to align the location of the two dipoles along $\er$. Given this formulation there are several interesting observations to make. First of all, $\FrBold$ and $\FtBold$ are attractive when $\alpha < \pi / 2$. Secondly the forces decline rapidly with the magnet-magnet distance: $1/d^4$. Given this large decay, actuation forces are limited to a shell around the device of roughly $d_{min} \leq d \lesssim d_{min} + 4cm$. $d_{min}=41mm$, since the radius of the sphere enclosure is $35.5mm$, the bottom layer in the tool is $2mm$ and the total volume height is $7mm$. 

\subsection{Calibration}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/calibrator.pdf}
    \caption{The calibration points used. The points are mirrored on the occluded side of the device. The total number of points is 36 of which 4 were discarded due to saturing an axis on a sensor. The device was a 3D printed shell, with holes at the highlighted locations.}
    \label{fig:my_label}
\end{figure}

In order for the cost term (Equation \ref{eq:eneregy} to work. The real world and model world hall sensor coordinates need to be sufficiently close. To answer the question: "how close is close enough?" we ran an experiment in which we evaluated the error of Algorithm \ref{algo:postion} over different errors in sensor position. Details can be found in Appendix \ref{appendix:analyse:calibration}. The result, shown in figure \ref{fig:calibration_accuracy_needed} seems to suggest that we need to know the position with less than 1mm accuracy. In order to achieve this, next to well designed hardware we need a calibration procedure. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/calibration_needed.pdf}
    \caption{Analyses on how precise we need to know the hall sensor location in 3D space. for different noise levels on sensor readings with regard to solve speed and accuracy. We use Alg. \ref{algo:postion} in simulation, however to the sensor reading $\mathbf{\Tilde{B}}$ are taken from a different initialization on sensor location in the model.}
    \label{fig:calibration_accuracy_needed}
\end{figure}

Another factor to consider is the gain of each sensor. This is the factor with which a reading needs to be multiplied, to get the real world value. The gain can be different between sensors, and also between axis on a sensor.

Our calibration procedure is similar, and based on the same foundation ,as the algorithm and physics we use for the tracking of a permanent magnet. In the tracking case, the sensor position is known and the magnet position is regressed to, in the calibration this is vice versa: the magnet position is known, but the sensors are not. Another difference is that we use ADAM to do update steps on our sensor positions, rather than the LBFGS algorithm. This is because solve time does not matter for calibration, and ADAM provided empirically better results.

We used 32 points on the surface of the sphere as calibration points. Theoretical a single point would suffice, however this decreases the noise in placement and in practice yields better results. For each magnet position we took a 1000 samples. From these samples we discarded the top and bottom 5\% and then used the mean of this sample, this was done per axis per sensor. This is done without the core present. 

\begin{algorithm}
\SetAlgoLined
\SetKwInOut{Output}{\textbf{Output}}
\SetKwInOut{Input}{\textbf{Input}}
\SetKwFunction{Alternate}{\textbf{Alternate}}
\KwResult{calibrated $x,y,z$-position of hall sensors}

 $\mathbf{S}\leftarrow \mathbb{R}^{n \times 3}$\tcp*{Initial estimate of hall sensor locations.}
 $\mathbf{C}\leftarrow x,y,z\text{-calibration positions} $\;
 $\mathbf{B}\leftarrow \text{sensor readings}$\;
 
 $\text{optimizer} \leftarrow \text{ADAM}$\;
 \While{Not Converged}{
  $\text{optimizer.params} \leftarrow \mathbf{S}$\;

     \While{Not Converged}{
        $loss \leftarrow 0$\;
        \For{$\mathbf{c},\mathbf{b} \in \text{zip}(\mathbf{C}, \mathbf{B}$)}{
            $\mathbf{b}_{\text{model}} \leftarrow \text{model}(\mathbf{c})$\;
            $loss += sum((\mathbf{b}_{\text{model}} - \mathbf{b})^2)$
        }
        $\text{loss.backprop()}$\;
        $\mathbf{S} \leftarrow \text{optimizer.step()}$\tcp*{take an update step on sensor location}
     }
 }
 \Output{$\mathbf{S}$}
 \caption{Hall Sensor Calibration}
 \label{algo:hall_Calibration}
\end{algorithm}

\subsection{Control}

From Eq \ref{eq:me_vs_I} follows:
\begin{equation}\label{eq:I_vs_me}
    \mathbf{I} = \mathbf{c} * \frac{\mathbf{m}_e * \mu_0}{2*\pi*\mathbf{d}^3} \quad ,
\end{equation}

\noindent here $\mathbf{c}$ is a constant coming from a calibration procedure; that, with the help of five hall sensors, maps input current to $\mathbf{m}_e$. $\mu_0=4*\pi*10^{-7}$ is the relative permeability of air and $d$ is the distance from the core to the hall sensors used for calibration ($0.055$ meter)


The magnetic field, and therefore the perceived force, follow Biot-Savart's law. This means that the magnetic is directly proportional to the current. We control the current Ohms Law:
\begin{equation}
    I = \frac{V}{R}
\end{equation}
If we know the resistance of the wire and, with Pulse-Width Modulation (PWM), control the voltage the current output directly follow.

Since we are using large amounts of current the whole system gets hot. This heat changes the resistance in the coils and we need to adapt our method accordingly. Previous worked use a PID controller to compensate for this overtime, however tuning PID controllers is cumbersome and even then would either lag in current supplied or oscillate. 

In order to overcome the unknown resitance of the coils we use sensors that can measure both current and voltage (INA260), again using Ohms law (and rewriting it), the resitance directly follows from both measurements. There we have an almost instantanously updating resistance of the coils. 


==> chapters/04_joint_interfaces/sensing/sections/06_applications.tex <==
\section{Applications}
We implemented a series of applications to showcase Omni's potential in supporting spatial interaction with virtual objects that is supported by strong haptic sensations as shown in Figure~\ref{fig:usecases}. While \textit{Omni} can support traditional desktop interaction with haptic cues (\eg free-form tool-based gesture input), we focus our applications on mixed and virtual reality scenarios that are inherently spatial.

Specifically, we demonstrate scenarios in MR, which benefit most from \textit{Omni}'s walk-up-and-use nature to track and haptically actuate an untethered, small magnet in the space around \textit{Omni}'s base.

We implemented our applications using a video pass-through Mixed Reality device (Varjo XR-1), shown in Figure~\ref{fig:photo_device_ar}.
\textit{Videos and photos were recorded live through Varjo's software.}
\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{\dir/sensing/figures/user-applications-live.pdf}
\caption{We combine \textit{Omni} with a video see-through MR device (Varjo XR-1) to showcase the applications.}
\label{fig:photo_device_ar}
\end{figure}

\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{\dir/sensing/figures/applications-02.jpg}
\caption{We present possible use cases for \textit{Omni}. \textit{Left} shows the possibilities in 3D CAD design, in this case sculpting. \textit{Center} shows a user exploring and manipulating an augmented reality object. For both applications, users can feel the shape of the outer hull of the objects. \textit{Right} shows a racing game. Once the car collides with the wall, the pen gets pushed to the base. \textit{Arrows indicate movement and are drawn on top of the photo to increase clarity}. }
\label{fig:usecases}
\vspace{-1em}
\end{figure*}

\subsection{Sculpting}
Figure~\ref{fig:usecases} illustrates how \textit{Omni} haptically supports 3D sculpting and CAD design.

Here, the user finely selects locations on a 3D base object for extrusion by means of the stylus, which is tracked through \textit{Omni}. When extruding individual bumps from the starting configuration, the user can probe and feel the compliance of the material, rendered through attractive and repulsive forces.
Having extruded several bumps from the original shape, the user may inspect the 3D object visually as well as haptically, as \textit{Omni} renders collisions with the tool through tangential actuation.

Following this 3D interaction scenario, \textit{Omni}'s haptic capabilities could be scaled to common 3D editing techniques such as grid snapping, guided object rotation, and 3D transformation.

\subsection{Non-rigid object exploration}
\textit{Omni}'s tracking and actuation also lends itself to haptically rendering geometric objects that are non-rigid and may have anisotropic material properties, such as geographical surfaces, enlarged microscopic surfaces, or other complex geometries.
We demonstrate how \textit{Omni} generates haptic feedback while touching and poking a virtual dragon that is configured to simulate rubber-like material properties.
Here, the force \textit{Omni} renders increases with the amount of object deformation, which portrays the \textit{physical behavior} more accurately than would be possible to experience through mere visual feedback.

\subsection{Gaming}
Finally, we demonstrate how \textit{Omni} can be used for enhancing the experience of gameplay.
Using the magnet-equipped tool as a joystick, we demonstrate how users can steer a car in an AR racing game.
The combination of \textit{Omni}'s haptic feedback and visual control over the car increases the level of immersion provided by the system, as haptic and visual sensations render a coherent experience.
For example, \textit{Omni} renders car collisions with forces whose magnitude depends on collision speeds.

==> chapters/04_joint_interfaces/sensing/sections/07_discussion.tex <==
\section{Discussion}
\omniUIST is capable of tracking a passive tool with an accuracy of roughly 6.9 mm and, at the same time, deliver a maximum force of up to 2 N to the tool. This is enabled by our novel gradient-based approach in 3D position reconstruction that accounts for the force exerted by the electromagnet. 

Over extended periods of time, \omniUIST can comfortably produce a force of 0.615 N without the risk of overheating. In our applications, we show that \omniUIST has the potential for a wide range of usage scenarios, specifically to enrich AR and VR interactions.

\omniUIST is, however, not limited to spatial applications. We believe that \omniUIST can be a valuable addition to desktop interfaces, e.g., navigating through video editing tools or gaming. We plan to broaden \omniUIST's usage scenarios in the future.

The overall tracking performance of \omniUIST suffices for interactive applications such as the ones shown in this paper. The accuracy could be improved by adding more Hall sensors, or optimizing their placement further (e.g., placing them on the outer hull of the device).
Furthermore, a spherical tip on the passive tool that more closely resembles the dipole in our magnetic model could further improve \omniUIST's accuracy. We believe, however, that the design of \omniUIST represents a good balance of cost and complexity of manufacturing, and accuracy.

Our current implementation of \omniUIST and the accompanying tracking and actuation algorithms assumes the presence of a single passive tool. Our method, however, potentially generalizes to tracking multiple passive tools by accounting for the presence of multiple permanent magnets. This poses another interesting challenge: the magnets of multiple tools will interact with each other, i.e., attract and repel each other.The electromagnet will also jointly interact with those tools, leading to challenges in terms of computation and convergence. We believe that our gradient-based optimization can account for such interactions and plan to investigate this in the future.

In developing and testing our applications, we found that \omniUIST's current frame rate of 40 Hz suffices for many interactive scenarios. The frame rate is a trade-off between speed and accuracy. In our tests, decreasing the desired accuracy in our optimization doubled the frame rate, while resulting in errors in the 3D position estimation of more than 1 cm, however. Finding the sweet spot for this trade-off depends on the application. While our applications worked well with 40 Hz and the current accuracy, more intricate actions such as high-precision sculpting might benefit from higher frame rates \textit{and} precision.
Reducing the latency of several system components (e.g., sensor latency, convergence time) is another interesting direction of future research. 

Furthermore, the control strategy we used was fairly naïve, as it only takes the current tool position into account. A model predictive strategy could account for future states, user intent, and optimize to reduce heating. We will explore in the next chapter how model predictive approaches can be used for haptic systems.

Overall, the main benefits of \omniUIST lie in the high accuracy and large force it can produce. It does so without mechanically moving parts, which would be subject to wear.
Such wear is not the case for our device, because it is exclusively based on electromagnetic force. We believe that different form factors of \omniUIST (e.g., body-mounted, larger size) can present interesting directions of future research. \add{A body-mounted version could be interesting for VR applications in which the user moves in 3D space. The larger size could result in more discernible points.}

Additionally, the influence of strength on user perception and factors such as just-noticeable-difference will allow us to characterize the benefits and challenges of \omniUIST, and electromagnetic haptic devices in general.
We believe that \omniUIST opens interesting directions for future research in terms of novel devices, and magnetic actuation and tracking.

==> chapters/04_joint_interfaces/sensing/sections/99_preamble.tex <==
% Use this section to set the ACM copyright statement (e.g. for
% preprints).  Consult the conference website for the camera-ready
% copyright statement.



% Use this command to override the default ACM copyright statement
% (e.g. for preprints).  Consult the conference website for the
% camera-ready copyright statement.

%% HOW TO OVERRIDE THE DEFAULT COPYRIGHT STRIP --
%% Please note you need to make sure the copy for your specific
%% license is used here!
% \toappear{
% Permission to make digital or hard copies of all or part of this work
% for personal or classroom use is granted without fee provided that
% copies are not made or distributed for profit or commercial advantage
% and that copies bear this notice and the full citation on the first
% page. Copyrights for components of this work owned by others than ACM
% must be honored. Abstracting with credit is permitted. To copy
% otherwise, or republish, to post on servers or to redistribute to
% lists, requires prior specific permission and/or a fee. Request
% permissions from \href{mailto:Permissions@acm.org}{Permissions@acm.org}. \\
% \emph{UIST '20},  October 20--23, 2020, Minneapolis, MN, USA \\
% ACM xxx-x-xxxx-xxxx-x/xx/xx\ldots \$15.00 \\
% DOI: \url{http://dx.doi.org/xx.xxxx/xxxxxxx.xxxxxxx}
% }

% Arabic page numbers for submission.  Remove this line to eliminate
% page numbers for the camera ready copy
%  \pagenumbering{arabic}

% Load basic packages
\usepackage{balance}       % to better equalize the last page
\usepackage{graphics}      % for EPS, load graphicx instead 
\usepackage[T1]{fontenc}   % for umlauts and other diaeresis
\usepackage{txfonts}
\usepackage{mathptmx}
\usepackage[pdflang={en-US},pdftex]{hyperref}
\usepackage{color}
\usepackage{booktabs}
\usepackage{textcomp}
\usepackage{graphicx,import}
\usepackage[caption=false]{subfig}
\usepackage[normalem]{ulem}

\usepackage{units}

\usepackage{textcomp}

% Some optional stuff you might like/need.
\usepackage{microtype}        % Improved Tracking and Kerning
% \usepackage[all]{hypcap}    % Fixes bug in hyperref caption linking
\usepackage{ccicons}          % Cite your images correctly!
% \usepackage[utf8]{inputenc} % for a UTF8 editor only

% If you want to use todo notes, marginpars etc. during creation of
% your draft document, you have to enable the "chi_draft" option for
% the document class. To do this, change the very first line to:
% "\documentclass[chi_draft]{sigchi}". You can then place todo notes
% by using the "\todo{...}"  command. Make sure to disable the draft
% option again before submitting your final document.
\usepackage{todonotes}
\usepackage[ruled,vlined]{algorithm2e}

% Paper metadata (use plain text, for PDF inclusion and later
% re-using, if desired).  Use \emtpyauthor when submitting for review
% so you remain anonymous.

% TITLE WORDS
% Volume
% Nonplanar
% Electromagnet
% Sphere
% Tracking
% Sensing
% Actuating
% untethered

%  Other paper: "Optimal Control for Electromagnetic Haptic Guidance Systems"

% \def\plaintitle{\systemname: Non-Planar Electromagnetic Haptic Feedback}
% \def\plaintitle{Electromagnetic Haptic Feedback Sensing and Actuating}
% \def\plaintitle{3 Degrees of Freedom Sensing and Actuation for Electromagnetic Haptic Feedback}
% \def\plaintitle{Volumetric Sensing and Actuation for Spherical Electromagnetic Haptic Feedback}
% \def\plaintitle{Sensing and Actuation for Electromagnetic Haptic Feedback}
% \def\plaintitle{Sensing and Actuation for Volumetric Electromagnetic Haptic Feedback}
% \def\plaintitle{Untethered Sensing and Actuation for Volumetric Electromagnetic Haptic Feedback}
% \def\plaintitle{Stand-Alone Sensing and Actuation for Electromagnetic Haptic Feedback}
% \def\plaintitle{Stand-Alone Sensing and Actuation for Electromagnetic Systems}

\def\plaintitle{Omni: Volumetric Sensing and Actuation of Passive Magnetic Tools for Dynamic Haptic Feedback}


\def\plainauthor{Thomas Langerack, Juan Jose Zarate, David Lindlbauer, Christian Holz, Otmar Hilliges}
\def\emptyauthor{}
\def\plainkeywords{Haptic feedback; Electromagnetic sensing; Electromagnets; Mixed Reality}
\def\plaingeneralterms{Documentation, Standardization}

% llt: Define a global style for URLs, rather that the default one
\makeatletter
\def\url@leostyle{%
  \@ifundefined{selectfont}{
    \def\UrlFont{\sf}
  }{
    \def\UrlFont{\small\bf\ttfamily}
  }}
\makeatother
\urlstyle{leo}

% To make various LaTeX processors do the right thing with page size.
% \def\pprw{8.5in}
% \def\pprh{11in}
% \special{papersize=\pprw,\pprh}
% \setlength{\paperwidth}{\pprw}
% \setlength{\paperheight}{\pprh}
% \setlength{\pdfpagewidth}{\pprw}
% \setlength{\pdfpageheight}{\pprh}

% Make sure hyperref comes last of your loaded packages, to give it a
% fighting chance of not being over-written, since its job is to
% redefine many LaTeX commands.
\definecolor{linkColor}{RGB}{6,125,233}
\hypersetup{%
  pdftitle={\plaintitle},
% Use \plainauthor for final version.
%  pdfauthor={\plainauthor},
  pdfauthor={\plainauthor},
  pdfkeywords={\plainkeywords},
  pdfdisplaydoctitle=true, % For Accessibility
  bookmarksnumbered,
  pdfstartview={FitH},
  colorlinks,
  citecolor=black,
  filecolor=black,
  linkcolor=black,
  urlcolor=linkColor,
  breaklinks=true,
  hypertexnames=false
}

==> chapters/05_shared_control/content/introduction.tex <==
\chapter{Introduction}
\label{ch:control:introduction}
% Problem --> Naive policy
In the previous part we have seen how haptic \interfaces might have the potential to increase the intuitiveness of interactions. However, our control strategy of the haptic actuators was na\"ive and not intelligent, leading to subpar interactions. Specifically, our control strategy was based around the current tool position and did not take into account user intent, future states of the system, or bounds to the control.  

% Solution --> Predictive
One solution to this problem is to make use of optimal control formulations (see \ref{}). Optimal control is a branch of control theory that deals with finding a control for a dynamical system over a period of time such that an objective function is minimized \cite{ross2015primer}. Although this addresses both the optimization over future states and enables constraints to the system, it does not take the user into account. 

% Our work
In contrast, our work enables explicit and implicit user models in optimal control strategies. To this end, we introduce two projects. First, we introduce \magpen. \magpen introduces an model predictive control method for electromagnetic haptic guidance systems. Our real-time approach assists users in pen-based tasks such as
drawing, sketching or designing. The key to our control method is that it guides users, yet does not take away agency. To achieve this flexible guidance, our optimization iteratively predicts the motion of an input device such as a pen, and adjusts the position and strength of an underlying dynamic electromagnetic actuator accordingly. However, \magpen relies on an explicit described linear system dynamic. This is challenging, as these system dynamic include a user model. We linearlized the user behavioral model through assumptions. However, this is suboptimal and does not generalize to other \interfaces. 

Second we introduce, \marlui. \marlui overcomes \magpen's limitation by learning system dynamics implicitly. In \marlui, we focus on adaptive user interfaces. Specifically, we formulate interface adaptation as a multi-agent reinforcement learning problem. Our approach learns adaptation policies without relying on heuristics or real user data, facilitating the development of adaptive interfaces across various tasks with minimal adjustments needed. In our formulation, a user agent mimics a real user and learns to interact with an interface via point-and-click actions. Simultaneously, an interface agent learns interface adaptations, to maximize the user agent’s efficiency, by observing the user agent’s behavior. 

% Implications
The implications of our research in shared control on \interfaces is two-fold. First, we show how to integrate models of human behavior explicitly and implicitly into optimal control strategies for intelligent systems. This enables the systems to take into account future states and actions, and optimize the system inputs accordingly. Second, we introduce a method that does not require an explicit user model or system dynamics description. This enables the method to generalize across interfaces and tasks. Treating HCI, and specifically the interaction with intelligent systems, as a multi-agent reinforcement problem is intuitive and enables future extensions of our work.  

% Summary
In summary, we introduce two optimal control strategies. First, A model-based predictive control strategy to optimize the input to a haptic system. Second, a model-free multi agent reinforcement learning strategy for adaptive user interfaces. We show that our methods enable an autonomy-automation trade-off, which results in better user performance, in terms of speed, accuracy and number of actions, compared to alternatives. Our research is a starting point to think and investigate the role of predictive user models in control loops. 

==> chapters/05_shared_control/mpc/sections/00_abstract.tex <==
% ABSTRACT DL V2
We introduce an optimal control method for electromagnetic haptic guidance systems. 
Our real-time approach assists users in pen-based tasks such as drawing, sketching or designing. 
The key to our control method is that it guides users, yet does not take away agency. 
Existing approaches force the stylus to a continuously advancing setpoint on a target trajectory, leading to undesirable behavior such as loss of haptic guidance or unintended snapping. 
Our control approach, in contrast, gently pulls users towards the target trajectory, allowing them to always easily override the system to adapt their input spontaneously and draw at their own speed. 
To achieve this flexible guidance, our optimization iteratively predicts the motion of an input device such as a pen, and adjusts the position and strength of an underlying dynamic electromagnetic actuator accordingly. 
To enable real-time computation, we additionally introduce a novel and fast approximate model of an electromagnet. 
We demonstrate the applicability of our approach by implementing it on a prototypical hardware platform based on an electromagnet moving on a bi-axial linear stage, as well as a set of applications. 
Experimental results show that our approach is more accurate and preferred by users compared to open-loop and time-dependent closed-loop approaches.

% ABSTRACT DL V1
% We introduce an optimal control method for electromagnetic haptic feedback systems.
% Our real-time approach enables assisting users in tasks such as drawing, sketching or designing \textit{without taking away agency}.
% Users can always easily override the system to adapt their trajectory.
% Our closed-loop time-free approach then gently pulls them back to the desired trajectory. 
% In contrast, existing approaches force the stylus to a continuously advancing setpoint, leading to undesirable behavior such as loss of haptic guidance or unintended snapping.
% To achieve this flexible guidance, our optimization only assumes a dynamic electromagnetic actuator underneath a drawing surface or display and an input device such as a stylus with an embedded permanent magnet. 
% We additionally introduce a novel fast and well-fitting approximate model of an electromagnet to enable real-time computation.
% We demonstrate the applicability of our approach by implementing it on a prototypical hardware platform based on an electromagnet moving on a bi-axial linear stage, as well as a set of applications.
% Experimental results show that our approach is more accurate and preferred by users compared to open-loop and time-dependent closed-loop approaches.


% Our experimental results show that the system can control the pen position with a very low dispersion of \unit[2.8]{mm} ($\pm$\unit[0.8]{mm}), and that our approach is more accurate and preferred by users compared to  open-loop and time-dependent closed-loop approaches.

==> chapters/05_shared_control/rl/sections/02_related.tex <==
%!TEX root = ../main.tex

\section{Related Work}
\label{sec:related}
This paper proposes multi-agent RL as a framework for adaptive UIs. Our method features a \useragent that models human interaction behavior and an \interfaceagent that adapts the UI to support the \useragent.
Most related to our work is research on computational user modeling, methods for adaptive UIs, and (MA)RL.

\subsection{Computational User Modelling}
Computational user modeling has a long tradition in HCI. These models predict user performance and are essential for UI optimization \cite{oulasvirta2018computational}. Early work relies on heuristics \cite{card1986model, card1980klm, card1983the, kieras1997overview, anderson1997act} and on simple mathematical models \cite{fitts1954information, hick1952rate}.
More recent work extends these models and, for instance, predicts the operating time for a linear menu \cite{10.1145/1240624.1240723}, gaze patterns \cite{salvucci2001integrated}, or cognitive load \cite{duchowski2018index}.

Recently, reinforcement learning gained popularity within the research area of computational user models.
This popularity is due to its neurological plausibility \cite{botvinick2012hierarchical, frank2012mechanisms}, allowing it to serve as a model of human cognitive functioning.
The underlying assumption of RL in HCI is that users behave rationally within their bounded resources \cite{gershman2015computational, oulasvirta2022computational}.
There is evidence that humans use such strategy across domains, such as in causal reasoning \cite{denison2013rational} or perception \cite{gershman2012multistability}.
In human-computer interaction, researchers have leveraged RL to automate the sequence of user actions in a KLM framework \cite{leino2019computer} or to predict fatigue in volumetric movements \cite{cheema2020predicting}.
It was also used to explain search behavior in user interfaces \cite{yang2020predicting} or menus \cite{chen2015emergence} and as a model for multitasking \cite{jokinen2021multitasking}.
Most similar to our work is research on hierarchical reinforcement learning for user modeling.
\citeauthor{jokinen2021touchscreen} \cite{jokinen2021touchscreen} show that human-like typing can emerge with the help of Fitts' Law and a gaze model.
Other works show that HRL can elicit human-like behavior in task interleaving \cite{gebhardt2020hierarchical} or touch interactions \cite{jokinen2021touchscreen}.
Inspired by this work, we design our user agent by decomposing high-level decision-making from motor control.
Using two hierarchical levels yields simulated behavior.

\subsection{Methods for Adaptive UIs}
UI adaptation can either be offline, to computationally design an interface, or online, to adapt the UI according to users' goals. We will focus on online adaptive UIs and refer readers to \cite{combinatorialoptimizationdesign2020oulasvirta, functionalityselection2017oulasvirta} for an overview of computational UI design.

\subsubsection{Heuristics, Bayesian Networks \& Combinatorial Optimization}
In early works, heuristic- or knowledge-based approaches are used to adapt the UI  \cite{Browne1990,Stephanidis1997,Smith2010}.
Similarly, multi-agent systems employ rule-based and message-passing approaches  \citep{Rich1998,Rich2005,Yorke2012}. Another popular technique for AUIs is domain-expert-designed Bayesian networks  \citep{Horvitz1998, Bosma2004}.
More recently, combinatorial optimization was used to adapt interfaces dynamically \cite{park2018adam, lindlbauer2019context}.
The downside of these approaches is that experts need to specify user goals using complex rule-based systems or mathematical formulations. 
Creating them comprehensively and accurately requires developers to foresee all possible user states, which is tedious and requires expert knowledge.
Commonly, these approaches also get into conflict when multiple rules or objectives apply.
This conflict often results in unintuitive adaptations.
In contrast, our method only requires the layout of the UI.
From its representation as an RL environment, we learn policies that meaningfully adapt the UI and realistically reproduce user behavior.

\subsubsection{\del{Machine Learning} \add{Supervised Learning}}
Leveraging machine learning can overcome the limitations of heuristic-, network-, and optimization-based systems by learning appropriate UI adaptions from user data.
Traditional machine learning approaches commonly learn a mapping from user input to UI adaptation. 
Algorithms like nearest neighbor  \cite{Maes1995, Lashkari1997}, Na\"ive Bayes  \cite{McCreath2006,Faulring2010}, perceptron \cite{Shen2009a, Shen2009b}, support vector machines \cite{Berry2011}, or random forests \cite{Pejovic2014, Mehrotra2015} are used and models are learned offline \cite{Berry2011} and online \cite{Shen2009a}.
Due to the problem setting, these approaches require users' input to be highly predictive of the most appropriate adaptation. 
Furthermore, it restricts the methods to work in use cases where myopic planning is sufficient, i.e., a single UI adaptation leads users to their goal. 
In contrast, our method considers multiple goals when selecting an adaptation and can lead users to their goal using sequences of adaptations. 

More recent work overcomes the limitations stemming from simple input-to-adaptation mapping by following a two-step approach. They (1) infer users' intention based on observations and (2) choose an appropriate adaptation based on the inferred intent \cite{oulasvirta2018computational}.
Such work uses neural networks, and user intention is modeled either explicitly \cite{kolekar2010learning, soh2017deep} or as a low-dimensional latent representation \cite{RIZZOGLIO2021}.
However, these approaches are still highly dependent on \deliui{the quality of the} training data, which may not even be available for emerging technologies. \deliui{In contrast, our method does not depend on pre-collected user data \emph{and} can learn supportive policies just by observing simulated user behavior. } \addiui{In contrast, our method can learn supportive policies without pre-collected user data by just observing simulated user behavior.}

\subsubsection{Bandits \& Bayesian Optimization} 
Bandit systems are a probabilistic approach often used in recommender systems \cite{glowacka2019bandit}.
In a multi-armed bandit setting, each adaptation is modeled as an arm with a probability distribution describing the expected reward.
The Bayes theorem updates the expectation, given a new observation and prior data.
Related work leverages this approach for AUIs \cite{lomas2016interface,koch2019may,kangas2022scalable}.
Bayesian optimization is a sample-efficient global optimization method that finds optimal solutions in multi-dimensional spaces by probing a black box function \cite{shahriari2015taking}. In the case of AUIs, it is used to find optimal UI adaptations by sampling users' preferences \cite{Koyama2014, Koyama2016}.
Both approaches trade off exploration and exploitation when searching for appropriate adaptations (i.e., exploration finds entirely new solutions, and exploitation improves existing solutions), rendering them suitable approaches to the AUI problem.

However, such methods are not able to plan adaptations over a sequence of interaction steps, i.e., they plan myopic strategies.
In addition, these approaches need to sample user feedback to learn or optimize for meaningful adaptations and, hence, also rely on high-fidelity user data.
Furthermore, as users themselves learn during training or optimization, solutions can converge to sub-optimal user behavior as such methods reduce exploration with convergence. 
In contrast, our method can plan adaptations over a sequence of interaction steps learned from realistic, simulated user data.  

\subsubsection{Reinforcement Learning} 
Reinforcement learning is a natural approach to solving the AUI problem, as its underlying decision-making formalism implicitly
captures the closed-loop iterative nature of HCI \cite{howes2018interaction}. 
It is a generalization of bandits and learns policies for longer horizons, where current actions can influence future states.
This generalization enables selecting UI adaptations according to user goals that require multiple interaction steps.
Its capability makes RL a powerful approach for AUIs with applications in dialog systems \cite{Gasic2014, Su2017}, crowdsourcing \cite{PengCrowdsourcing2013, Hu2018}, sequential recommendations \cite{Chen2019, Liu2018, Liebman2015}, information filtering \cite{seo2000reinforcement}, personalized web page design \cite{ferretti2014exploiting}, and mixed reality \cite{gebhardt2019learning}.
Similar to our work is a model-based RL method that optimizes menu adaptations \cite{todi2021adapting}.

Current RL methods sample predictive models \cite{todi2021adapting, Gasic2014, Hu2018} or logged user traces  \cite{gebhardt2019learning}. However, these predictive models and offline traces represent user interactions with non-adaptive interfaces. Introducing an adaptive interface will change user behavior; so-called co-adaptation \cite{mackay2000responding}. Hence, it is unclear if the learned model can choose meaningful adaptations when user behavior changes significantly due to the model's introduction. In contrast, our user agent learns to interact with the adapted UI; hence, our interface agent learns on behavioral traces from the adapted setting.

\subsubsection{Multi-Agent Reinforcement Learning}
MARL is a generalization of RL in which multiple agents act, competitively or cooperatively, in a shared environment \cite{zhang2021multi}.  
%
Multi-agent systems are common in games \cite{baker2019emergent, jaderberg2019quake}, robotics \cite{ota2006multiagent,sariff2018multiagent}, or modeling of social dilemmas \cite{chao2015social,leibo2017multi}. MARL is challenging since multiple agents change their behavior as training progresses, making the learning problem non-stationary. Common techniques to address this issue is via implicit \cite{tian2020implicit} or explicit \cite{foerster2016learning} communication, centralized critic functions \cite{lowe2017multi,yu2021surprising}, or curricula \cite{epciclr2020,wang2020curriculum}. We take inspiration from the latter and use a curriculum during the training of our agents.

Closest to our work is \cite{debard2020multiagent}, which proposes a multi-agent system that maps 2D interface trajectories to actions for navigating 3D virtual environments. A user agent learns interactions on a 2D interface. A decoder that is trained on real user data maps the user agent's actions to 2D touch gestures. A second agent then translates these 2D touch gestures into 3D operations. 
In their setting, the interface agent does not observe the environment itself but receives the actions of the user agent as its state.
Our work extends their setting to the case where the user agent and the interface agent observe and manipulate the same UI. Furthermore, we do not rely on real world user data.


==> preamble/_cv.tex <==
%*******************************************************
% CV
%*******************************************************
\pdfbookmark[1]{Curriculum Vitae}{cv}

\bigskip

\begingroup
\let\clearpage\relax
\let\cleardoublepage\relax
\let\cleardoublepage\relax
\chapter*{Curriculum Vitae}

\section*{Personal data}

\noindent\cvleft{Name}%
\cvright{Thomas Langerak}\\
%
\cvleft{Date of Birth}%
\cvright{January 13, 1994}\\
%
\cvleft{Place of Birth}%
\cvright{Nieuwegein, the Netherlands}\\
%
\cvleft{Citizen of}%
\cvright{the Netherlands}

\section*{Education}

\noindent\cvleft{2016 --~2018}%
\cvright{%
  Aalto University \\
  Espoo, Finland\\
  \emph{Final degree:} Master of Science
}\vspace{0.75em}


\noindent\cvleft{2016 --~2018}%
\cvright{%
  University of Twente \\
  Enschede, the Netherlands\\
  \emph{Final degree:} Master of Science
}\vspace{0.75em}


\noindent\cvleft{2012--2016}%
\cvright{%
  Technische Universiteit Eindhoven\\
  Eindhoven, the Netherland\\
  \emph{Final degree:} Bachelor of Science
}\vspace{0.75em}

\noindent\cvleft{2006-~2012}%
\cvright{%
  Cals College (High School)\\
  Nieuwegein, the Netherlands
}

\endgroup

